Free2Shard: Adaptive-adversary-resistant sharding via Dynamic Self Allocation

Propelled by the growth of large-scale blockchain deployments, much recent progress has been made in designing sharding protocols that achieve throughput scaling linearly in the number of nodes. However, existing protocols are not robust to an adversary adaptively corrupting a fixed fraction of nodes. In this paper, we propose Free2Shard -- a new architecture that achieves near-linear scaling while being secure against a fully adaptive adversary. The focal point of this architecture is a dynamic self-allocation algorithm that lets users allocate themselves to shards in response to adversarial action, without requiring a central or cryptographic proof. This architecture has several attractive features unusual for sharding protocols, including: (a) the ability to handle the regime of large number of shards (relative to the number of nodes); (b) heterogeneous shard demands; (c) requiring only a small minority to follow the self-allocation; (d) asynchronous shard rotation; (e) operation in a purely identity-free proof-of-work setting. The key technical contribution is a deep mathematical connection to the classical work of Blackwell in dynamic game theory.

==> CMT.tex <==
\section{Data availability engine}

\label{sec: DA_CMT}

NO LONGER IN USE

Data availability is an important problem with sharding since we cannot expect any peer to check if all shard blocks in the total ordered log are available to honest peers in their respective shards, since the communication becomes prohibitively expensive as the number of shards and the total throughput grows. To achieve full decentralization, we would like to keep the communication load at each peer almost constant as the number of shards increases. 

As such motivated, we phrase the following \emph{data availability} problem: Given only the header of some shard block ${\bf B}$ in shard $i$, how can a peer maintaining the consensus engine verify that the data is available with at least one honest peer in shard $i$ in a {\em communication efficient} manner? More specifically, any protocol to verify data availability should satisfy the security requirements of \textbf{Soundness} and \textbf{Agreement} as defined in section \ref{sec:general}.

We solve the above data availability problem %and scale the communication of 
by utilizing coded Merkle tree (CMT)~\cite{CMT}, which is a technique for a light node who only stores block headers to verify the data availability in a communication-efficient manner. Specifically, to apply CMT, we make a minimal assumption that each peer is connected to {\em at least one honest peer in every shard},\footnote{Note that this assumption is much weaker than assuming that majority of each shard is honest.} and a peer maintaining consensus engine is viewed as a light node to shard $i$ for every shard except the peer's own.

\subsection{Efficient random sampling via erasure coding}
Instead of downloading the entire block, a consensus peer could randomly sample a small portion of ${\bf B}$, from some peer in shard $i$ who claims to have the entire ${\bf B}$. It was proposed in~\cite{al2018fraud} to do this efficiently using erasure codes (see, e.g.,~\cite{lin2001error}). For the purpose of data availability, we can view ${\bf B}$ as a stream of $b$ bytes. For some design parameter $p$, we can evenly and arbitrarily partition the block into $p$ data symbols $w_1,\cdots,w_p$. The block producer encodes ${\bf B}$ into $n \geq p$ coded symbols $c_1,\cdots,c_n$ using e.g., an $(n,p)$ Reed-Solomon (RS) code. In this case, ${\bf B}$ can be recovered using {\em any} $p$ out of $n$ coded symbols, and it is available unless $n-p+1$ coded symbols are missing. When for instance $n=2p$, as illustrated in Fig.~\ref{fig:block-coding}, 
after successfully sampling $S$ coded symbols, a node in shard $i$ gains confidence that with probability $1-(\frac{p-1}{2p})^S$ some node in shard $j$ has at least 50\% of the coded symbols so it can completely recover ${\bf B}$. 
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/block-coding.pdf}
    \caption{Random sampling to check data availability of a block ${\bf B}$, which is encoded by a $(2p,p)$ Reed-Solomon code.}
    \label{fig:block-coding}
    \vspace{-5mm}
\end{figure}

While a consensus peer knows that some peer in shard $i$ will have sufficiently many symbols to decode, it cannot verify that the coding was done correctly and the decoded block is indeed the original ${\bf B}$. To defend such ``incorrect-coding'' fraud, the nodes outside the shard will forward their sampled symbols to their neighbouring nodes inside the shard, and rely on them to detect coding errors.

\noindent {\bf Coding-fraud proof.} An honest peer in shard $i$ decodes the block ${\bf B}$, and verifies the correctness of coding by comparing the Merkle root committed to the decoded block with the one stored in the header. Upon a mismatch, the node constructs a coding-fraud proof to inform the other nodes in shard $i$. %, so they can safely ignore this transaction block when constructing the ledger. 
This proof, as large as the original block, contains $p$ coded symbols using which ${\bf B}$ can be decoded and verified. It was proposed in~\cite{al2018fraud} to use 2-dimensional Reed-Solomon (2D-RS) codes to reduce the proof size from $b$ to $\sqrt{b}$, at the cost of storing $2\sqrt{n}$ additional hashes in the header.

In our protocol, a coding-fraud proof is published as a special entry on the total order log. Since each entry on the total order log is downloaded by every node in the network, %when the size of a shard transaction block scales with the number of shards $K$, the communication cost at a single node to download the proof for a 2D-RS code %generated according to~\cite{al2018fraud} will scale as $O(\sqrt{K})$. Hence, 
to make our protocol communication efficient, we need a mechanism to verify data availability with 1) constant sampling size for shard blocks, and 2) constant coding-fraud proof size.  

\subsection{Constant communication via coded Merkle tree}

\textbf{Optional start}
An $(n,p)$ linear code is characterized by a $(n-p) \times n$ parity check matrix ${\bf H}$, such that a transaction block is correctly encoded iff the coded symbols $c_1,\ldots,c_n$ satisfies ${\bf H} [c_1,\cdots,c_n]^\top = {\bf 0}$. In other words, the coded block has to pass $n-p$ parity check equations, each of which is an inner product with a row of ${\bf H}$. Since an incorrectly encoded block fails at least one equation, we propose to use a {\em single} failed equation as the coding-fraud proof. 

To make this proof succinct, we leverage low-density parity-check (LDPC) codes for which each parity check equation involves computing XOR of a \emph{constant} number of $d$ symbols. When one of the equations is violated, the decoder generates a coding-fraud proof consisting of $d-1$ symbols and $d$ membership proofs for all the symbols in that equation. Another node can easily verify the proof by 1) checking that the $d-1$ symbols pass their membership proofs, and 2) decoding the missing symbol, and verifying that it fails its membership proof. To enable such a  proof, our protocol adopts a hash-aware peeling decoder, which decodes a new symbol from an equation with $d-1$ hash-verified symbols at each time.

We use LDPC ensembles that are known to perform well under the peeling decoder (see, e.g.,~\cite{orlitsky2005stopping}), i.e., the ones with large ``stopping distance" which are guaranteed to be decodable even if only a constant fraction of the coded symbols are available. As an example, an $(n,p) = (32000,8000)$ regular LDPC code whose parity check equation involves $d = 8$ coded symbols can be decoded by a peeling decoder from any $0.876n = 28032$ symbols, with probability of at least $99.97\%$. This also makes the probability that the block is not available, but not detected by a node after $S = 30$ samples as small as $0.00063\%$. Therefore, a node outside the shard takes a constant number of samples to check data availability.

To be able to identify which equation is violated during peeling decoding, we require the hash commitments of \emph{all} coded symbols available at the decoder. Storing all of them in the block header is prohibitively expensive since the number of hashes increases with block size $n$. To resolve this issue, we choose to recover the hashes on-the-fly, by utilizing coded Merkle tree (CMT)~\cite{CMT}, which iteratively encodes the data with an LDPC code, computes hash commitments of the coded symbols, and concatenates these hashes into the data for the next level, until the size of the hash commitments is small enough to be stored in the block header. 

\textbf{Optional end}

\noindent {\bf Brief description of CMT.} The first level of the tree consists of $n$ coded symbols, created from $p$ data symbols constituting the original block via a rate $r = p/n$ systematic LDPC code. For the second level, we first compute the hashes of all the symbols in the first level, then aggregate $q \geq 2$ hashes together to form a total of $n/q$ new data symbols, and then use another $(\frac{n}{qr},\frac{n}{q})$ LDPC code to generate $\frac{n}{qr}$ coded symbols. We repeat this process to grow higher levels of the tree, until reaching a constant target number of $t$ hashes, which are stored in the header.\footnote{A standard Merkle tree is a special case of CMT  with $r=1$, $q=2$, and $t=1$.} %See Fig.~\ref{fig:coded_Merkle_tree} for an example where $k=16$, $r = \frac{1}{2}$, $q = 4$, and $t=4$. 
The membership proof of a base level symbol in CMT consists of all the sibling hashes between this symbol and the tree root, and the proof automatically provides membership proofs for all the symbols on the higher levels in the proof. Hence, sampling a symbol on the base level samples one membership-proved symbol on each level of CMT for free. %Interested readers are referred to~\cite{CMT2019}, for further details on the selections of LDPC codes on each level, and the exact construction of CMT.  

To decode a block, a node decodes the corresponding CMT starting from the top level, and all the way down to the base level. The decoded data at each level, which is the hash commitments of the symbols on the level below, is used to verify the symbols that are newly decoded from the peeling decoder. This allows a node to construct a coding-fraud proof at any level with a constant size of $d-1$ symbols. 

% Using CMT, the constant storage and computation of \tf at each node is maintained since 1) each block stores a constant number of CMT root hashes in the header, 2) the decoding complexity of a peeling decoder is linear in block size. 

\noindent {\bf Constant communication load.}
%As we mention before, using a peeling decoder for an LDPC code achieves high sampling efficiency, such that each node only needs to sample a constant number of symbols before detecting the unavailability of a block. 
Let us say for the LDPC codes used in CMT a constant $\alpha$ fraction of the coded symbols need to be received to decode the block, and each node randomly samples a constant number of $S$ symbols uniformly at random. Then on average we will need samples from $N = \frac{\alpha n }{S\log(1-\alpha)} \approx O(n)$ peers. Therefore, the number of symbols in each block $n$ also scales with the network size $N$. For a fixed target throughput in a single shard, scaling up the size of a block makes the block generation rate scale as $O(\frac{1}{N})$. Now, let us consider the communication load at a node that consists of two parts:
\begin{itemize}
    \item Sampling cost: it takes $S$ symbols from each of the transaction blocks in the $K-1 = \Theta(N)$ foreign shards. This leads to a constant $O(\frac{S (K-1)}{N}) = O(1)$ communication rate.
    \item Coding-fraud proof cost: it downloads $d-1$ symbols for each coding-fraud proof from a shard, which incurs a total communication rate of $O(\frac{(d-1)K}{N}) = O(1)$.  
\end{itemize}
This demonstrates that our protocol is communication-efficient, and the bandwidth consumption at each node remains constant as the number of shards increases. %We show that \tf with CMT based data-availability is secure in Appendix \ref{sec:cmt_security}

\textbf{Optional security guarantees}

==> algorithms.tex <==
\section{Algorithms}
\label{app:alg}
\subsection{Trifecta LC Miner}
\begin{algorithm}
{\fontsize{8pt}{8pt}\selectfont
\caption{\tflc Miner}\label{alg:miner}
\begin{algorithmic}[1]

\Procedure{Main()}{}
\State \textsc{Initialize()}
\While{true}
\State $(header,proposerCont,shardCont)$ = \textsc{PowMining()}
\If{$header$ is a $proposer$ $block$}
\State $block$ $\leftarrow$ $(header, proposerCont)$
\ElsIf{$header$ is a $shard$ $block$}
\State $block$ $\leftarrow$ $(header, shardCont)$
\EndIf
\State \textsc{BroadcastMessage($block$)}
\EndWhile
\EndProcedure
\vspace{2mm}
\Procedure{Initialize()}{}
\State $proposerTree$ $\leftarrow$ $proposerGenesis$
\State $proposerParent$ $\leftarrow$ $proposerGenesis$
\State $shardBlkDb$ $\leftarrow$ $\phi$ \colorcomment{shard blocks database}
\State $unRefShardBlksPool$ $\leftarrow$ $\phi$ \colorcomment{proposer block content}
\State $shardTxPool$ $\leftarrow$ $\phi$ \colorcomment{shard block content}
\EndProcedure
\vspace{2mm}

\Procedure{PowMining()}{} \label{code:pow_start}
\While{true}
\State $nativeShardId$ $\leftarrow$ $s$ \colorcomment{node chooses its own shard}
% \State $proposerCont$ $\leftarrow$ $proposerTxPool$
% \State $shardCont$ $\leftarrow$ $shardTxPool$
% \State $unRefShardPtrs$ $\leftarrow$ $unRefShardBlksPool$
\State $proposerCntMT$ $\leftarrow$ $MerkleTree(unRefShardBlksPool)$
\State $shardCntMT$ $\leftarrow$ $MerkleTree(shardTxPool)$
\State $nonce$ $\leftarrow$ $randomString$
\State $header$ $\leftarrow$ $(nonce,\; nativeShardId,\; proposerParent,$
\State $\qquad\qquad\qquad proposerCntMT.root,\; shardCntMT.root)$
\If {Hash(header)  $\leq \tau_1$} \colorcomment{proposer block mined}
    \State \textit{break}
\ElsIf{ $\tau_1 \leq $ Hash(header)  $\leq \tau_2$} \colorcomment{shard block mined}
    \State \textit{break}
\EndIf
\EndWhile
\Return $(header,proposerCont,shardCont)$ \label{code:pow_end}
\EndProcedure
\vspace{2mm}
\Procedure{ReceiveBlock($B$)}{}
\State \textsc{CheckPoW(B)}
\If{$B$ is a proposer block}
\If{$B.proposerCont \subseteq shardBlkDb$ }
\If {$proposerParent = B.proposerParent$} \colorcomment{mined on longest chain}
\State $proposerTree$.add($B$)
\State $proposerParent \leftarrow B$  \colorcomment{advancing the mining tip}
\State $unRefShardBlksPool$.remove($B.proposerCont$)
\ElsIf{$B.proposerParent \not\in proposerTree$ }
\State \textsc{RequestNetwork}($B.proposerParent$)
\Else \colorcomment{orphan block}
\State $proposerTree$.add($B$)
\EndIf
\ElsIf{$B.proposerCont \not\subseteq shardBlkDb$}
\State \textsc{RequestNetwork}($B.proposerCont \setminus shardBlkDb$)
\EndIf
\ElsIf{$B$ is a shard block}
\State $shardBlkDb$.add$(B)$
\If{$B.ShardId=nativeShardId$}
\State $shardTxPool$.remove($B.shardCont$)
\EndIf
\State $unRefShardBlksPool$.append($B.hash$)
\EndIf
\State \textsc{NetworkForward(B)}
\EndProcedure
\vspace{2mm}
\Procedure{ReceiveTx($tx$)}{}
\If{$tx.type$ = proposer}
\If{$tx$ is valid} proposerTxPool.append($tx$)
\EndIf
\ElsIf{$tx.type$ = shard AND $shardId=k$}
\If{$tx$ has valid signature}  shardTxPool.append($tx$)
\EndIf
\EndIf
\EndProcedure
\end{algorithmic}
}
\end{algorithm}

==> archive/del1.tex <==
These sharding protocols justify the safety and liveness attack by assuming that the adaptive adversary is slower that the periodic rate at which N2S allocation is called which is very powerful assumption since adversaries can typically be assumed faster than honest nodes.
Ethereum Serenity and Polkadot try to fend-off the safety vulnerability by introducing state transition validity fraud proofs \cite{teutsch2019scalable} for state commitments; however, this does not solve the liveness vulnerability and safety vulnerability between state commitments.

Let us assume a timescale where the consensus engine confirms one block per unit time. Let us assume that the miners for a shard $i$ mine a block with a rate of $r_i(t)$, the shard block mining power of honest miners in the shard is $\gamma_i(t)$ and the mining power of adversarial miners in $\beta_i(t)$, with 
\begin{align}
    \sum_{j=1}^K \gamma_j(t) = \gamma = 1-\beta = 1 - \sum_{j=1}^K \beta_j(t)
\end{align}

The number of honest and adversarial blocks mined in [t-1,t] is given by $R_i(t)\gamma_i(t)$ and $R_i(t)\beta_i(t)$ respectively. These blocks will be referred by the next consensus engine block at time $t$. The total number of shard $i$ blocks referred by the consensus block at time $t$ is constant $R$, i.e. $R_i(t)\gamma_i(t)+ R_i(t)\beta_i(t) = R$. Thus, the number of honest blocks added to the ledger of shard $i$ is denoted by $R\frac{\gamma_i(t)}{\gamma_i(t) + \beta_i(t)}$, we denote the normalized version with $R=1$ as the throughput $r_i(t)$ of shard $i$ at time $t$ denoted by:
\begin{align}
    r_i(t) &= \frac{\gamma_i(t)}{\gamma_i(t) + \beta_i(t)} \\
    \bar{r}(t) &= \frac{1}{t}\sum_{j=1}^t r_i(j)
\end{align}

We consider a trivial self-allocation scheme where honest nodes allocate themselves uniformly to one of $K$ shards. This distribution ensures that $\gamma_i(t) = \frac{\gamma}{K} \forall i \in [K]$. Consider an adversary which targets shard $1$ and throttles its throughput by allocating all its mining power to this shard, thus $\beta_1(t)=\beta$. This renders the throughput of shard 1 as $\frac{\gamma/K}{\gamma/K + \beta} = O(1/K)$. Thus, the throughput of the shard being attacked approaches 0 as number of shards ($K$) increases. 

This attack is fatal to the liveness of the shard since the adversary can censor honest transactions, the shard can no longer process most($O(1-1/K)$) of the honest transactions it receives since only $O(1/K)$ of transactions can be posted on the total ordered log.

%The \tfp architecture is summarized in figure \ref{fig:overview} and consists of the following 2 black boxes in addition to the uniconsensus architecture:
\begin{itemize}
    \item \textbf{Dynamic self-allocation engine}: Responsible for suggesting allocation of a shard to a node. Honest node calls at time intervals of unit length
    \textit{Input}: Total order log.
    \textit{Output}: Suggested shard to maintain
    \textit{Properties}: $\bar{r}_i(t)>h \forall i \in [K]$ where $h$ is a constant independent of $K$.
    \item \textbf{State commitment engine}: Similar i/o to ones defined in multi-cast architecture, internal working different due to uniconsensus architecture.
\end{itemize}

\begin{itemize}
    \item Set constants $c,b,q=b/(1-2b),s=\min(K, \frac{N}{\log N}), h=(1 - s e^{-nc\frac{b}{s}\log(c)})c(1-2b)\frac{s}{K}\gamma$ such that $h$ is as close to $\gamma$ as desired
    \item Set $u_i(t-1) = (h-\bar{r}_i(t-1))^+$
    \item Compute $\tilde{u_i}(t-1) = u_i(t-1)$ if $u_i$ is in the highest $s$ in $\boldsymbol{u(t-1)}$ and 0 otherwise
    \item Let $\tilde{\gamma}_i = \gamma \frac{\tilde{u}_i}{\sum_{i=1}^K \tilde{u}_i}$, compute $\boldsymbol{\gamma} = \frac{1}{1+q/\gamma} \underset{C_{q/s}}{\rm Proj} \, \boldsymbol{\tilde{\gamma}}$.
\end{itemize}



\paragraph{Blackwell similarity:} The motivation of the current approach comes from Blackwell approachability theorem which states that if the following conditions hold:
\begin{align}
    \forall \boldsymbol{\beta} \: \exists \boldsymbol{\gamma} \: s.t \: r(\boldsymbol{\gamma},\boldsymbol{\beta}) &\in C_h \label{eqn:blackwell_cond1}\\
    \text{For all half-spaces H containing $C_h$, } &\exists \boldsymbol{\gamma}\: s.t \: \forall\boldsymbol{\beta}\: , r(\boldsymbol{\gamma},\boldsymbol{\beta}) \in H \label{eqn:blackwell_cond2}
\end{align}

then there exists an adaptive strategy $f_t$ such that $\forall \boldsymbol{\beta(1)}, \boldsymbol{\beta(2)}, ..$
\begin{align}
    d\left( \frac{1}{T} \sum_{t=1}^T \boldsymbol{r}(\boldsymbol{\gamma(t)},\boldsymbol{\beta(t)}),C_h \right) \rightarrow 0
\end{align}

where $d$ is the usual euclidean distance metric on $\mathbb{R}^K$ extended to $\mathbb{R}^K \text{X} 2^{\mathbb{R}^K}$ by $d(x,C_h) = \inf_{s\in C_h} d(x,s)$

We observe that condition 1 represented by \eqref{eqn:blackwell_cond1} is satisfied by setting $\boldsymbol{\gamma} = \frac{\gamma}{\beta}\boldsymbol{\beta}$ and $h=\gamma$. We can also show that condition 2 (see \eqref{eqn:blackwell_cond2}) is satisfied by a honest policy $\boldsymbol{\gamma}$. However, we deviate from the Blackwell approachability result due to the stochastic nature of the honest action $\boldsymbol{\Gamma}$ which leads to $\mathbb{E}_{\boldsymbol{\Gamma}}[r_i(t)] \neq \frac{\gamma_i(t)}{\gamma_i(t)+\beta_i(t)}$.

\begin{figure}
    \centering
    \includegraphics[width = .4\textwidth]{images/dsa1.pdf}
    \caption{Simple DSA policy (eq:\ref{eq:simpledynamic}), adversary gradually attacks shard 1, and honest nodes follow it with a delay of one round, the attack is reset when the adversary has allocated all it's  power to shard 1}
    \label{fig:dsa1}
\end{figure}

==> archive/dynamicSA_old.tex <==
\section{Dynamic Self Allocation engine}

Our protocol allows peers to join any shard they want without any central consensus engine guiding them. We discussed in section \ref{sec:relwork} that following a trivial self allocation policy leads to a liveness attack. We then propose a few policies that solve the problem, with our final policy ensuring that independent non-coordinating honest peers can completely nullify the effects of a coordinating adversary within a constant factor $h$.

We follow the notion of throughput as defined in section \ref{sec:relwork}. Let $\gamma_i(t)$ and $\beta_i(t)$ denote the target honest and adversarial normalized mining power at shard $i$ at time $t$ and $\Gamma_i(t)$ and $B_i(t,\boldsymbol{\Gamma(t)})$ denote the actual honest and adversarial mining power allocated to the shard $i$ at time $t$, and let $\gamma$ and $\beta$ denote the total honest and adversarial normalized mining power. These target variables obey the following constraints:
\begin{align}
    \sum_{i=1}^K \gamma_i(t) &= \gamma \\
    \sum_{i=1}^K \beta_i(t) &= \beta \\
    \gamma + \beta = 1
\end{align}
Notice that we define target and actual variables separately since there are only $n=N\gamma$ honest peers in the network and each peer joins a shard with a probability $\gamma_i(t)$, thus $\Gamma_i(t)$ is a random variable defined as follows:
\begin{align}
    \Gamma_i(t) &= \frac{1}{N} \mathit{Binomial}(n,\gamma_i(t))
\end{align}
notice that the actual adversarial mining power in shard $i$ is $B_i(t,\boldsymbol{\Gamma(t)})$ since we assume that the adversary can optimize after looking at honest peer distribution and can split an adversarial peer between multiple shards.

Let $r_i(t)$ denote the instantaneous throughput of a shard $i$ at time $t$ and $\bar{r}_i(t)$ denote the average throughput of shard $i$ averaged from genesis($t=0$) till time $t$. Let $\mathbf{r}(t) = [r_1(t), r_2(t), .., r_K(t)]$ and $\mathbf{\bar{r}}(t) = [\bar{r}_1(t), \bar{r}_2(t), .., \bar{r}_K(t)]$ denote the corresponding vectors encompassing all the $K$ shards. We can define the instantaneous and average throughput in terms of the honest and adversarial mining power in a shard as follows:
\begin{align}
    r_i(t) &= \frac{\Gamma_i(t)}{\Gamma_i(t)+B_i(t,\boldsymbol{\Gamma(t)})}\\
    \bar{r}_i(t) &= \frac{1}{t} \sum_{i=1}^{t} r_i(t)
\end{align}

We organize this section by showing an attack on the trivial self allocation protocol and a DSA policy that can improve on the trivial protocol. We assume a fluid model during this subsections for ease of  understanding. We conclude this section by introducing a DSA policy that ensures that independent non-coordinating honest peers can completely nullify the throttling effects of a coordinating adversary within a constant factor. We analyze the final policy in a stochastic setting with a finite number of nodes $N$. We show that our final DSA policy works even for $N<K$.

\subsection{Throughput throttling attack}

We consider a trivial self-allocation scheme where honest nodes allocate themselves uniformly to $K$ shards. This distribution ensures that $\gamma_i(t) = \frac{\gamma}{K} \forall i \in [K]$. Consider an adversary which targets shard $1$ and throttles its throughput by allocating all its mining power to this shard, thus $\beta_1(t)=\beta$. This renders the throughput of shard 1 as $\frac{\gamma/K}{\gamma/K + \beta} = O(1/K)$. Thus, the throughput of the shard being attacked approaches 0 as number of shards ($K$) increases. 

This attack is fatal to the liveness of the shard since the adversary can censor honest transactions, the shard can no longer process most($O(1-1/K)$) of the honest transactions it receives since only $O(1/K)$ of transactions can be posted on the total ordered log. An example of this attack is shown in figure \ref{fig:tp_suppression}. 

\begin{figure}
    \centering
    \includegraphics[width = .48\textwidth]{images/tp_suppression_1.pdf}
    \caption{Throughput suppression}
    \label{fig:tp_suppression}
\end{figure}

We define the main optimization objective function which tries to find the optimal honest strategy that can achieve a worst case shard throughput of $\psi(K)$ given any adversarial strategy:
\begin{equation}
   \psi(K) = \max_{\{f_t\}_t} \, \min_{\{\beta_i(t)\}_{i,t}} \, \min_i \left\{ \frac{1}{T} \sum_{t=1}^T \frac{\gamma_i(t)}{\gamma_i(t)+\beta_i(t)} \right\} \label{eqn:main_function}
\end{equation}



\subsection{\dsaa}

We introduce \dsaa dynamic self allocation algorithm that ensures that the worst case average throughput of any shard is $O(1/log(K))$. 
The DSA algorithm specifies for each $t$, a function $f_t$ as follows:
\begin{equation}
  f_t: (\vec{\beta}(1),...\vec{\beta}(t-1),\vec{\gamma}(1),...\vec{\gamma}(t-1)) \rightarrow \vec{\gamma}(t)
\end{equation}
satisfying the constraint $\sum_i \gamma_i(t) = \gamma$.

We define $\psi_{f_t}(K)$: the throughput of the worst performing shard under a worst case adversary as follows:
\begin{equation}
   \psi_{f_t}(K) = \, \min_{\{\beta_i(t)\}_{i,t}}    \, \min_i \left\{ \bar{r}_i(t) \right\} 
\end{equation}
Note that the adversary at time $t$ has the knowledge of honest policy at time $t$.

The \dsaa algorithm specifies $f_t$ as follows:
\begin{align}
    f_{t} := {\gamma_i}(t) =    \{ \frac{\gamma}{2\beta} \beta_i(t-1) + \frac{\gamma}{2K} \} 
\end{align}

\begin{theorem}
    \dsaa algorithm ensures that the throughput of the worst performing shard for an optimal adversary lies within the range: $\Omega\left(\frac{1}{\log K}\right) \leq \psi_{f_{t}}(K)  \leq O \left(\frac{\log \log K}{\log K} \right)$
    \label{thm:dsa1}
\end{theorem}

\begin{proof}
    We provide a brief description of the proof below, Please refer to section \ref{sec:proof} for the detailed proof. We first prove a lower bound on the throughput by showing that any adversarial policy cannot maintain a throughput lower than a threshold $g$ for more than $\tau$ rounds, both a function of $K$.
    The upper bound is derived by showing that we can design an adversarial strategy than can achieve $O(\frac{log (K)}{log (log(K))})$ throughput. The adversarial strategy consists of increasing the adversarial mining power in a shard by a constant fraction and initiating a reset when a maximum adversarial mining power is allocated to the target shard.
\end{proof}

An example of an adversarial attack on shard 1 which renders a throughput of $O(\frac{log(K)}{log(log(K))})$ is shown in figure \ref{fig:dsa1}
\begin{figure}
    \centering
    \includegraphics[width = .4\textwidth]{images/dsa1.pdf}
    \caption{\dsaa example}
    \label{fig:dsa1}
\end{figure}

We observe that this simple algorithm of following the adversarial distribution of the past time instant improves the worst case shard throughput from $O(1/K)$ to $O(1/log(K))$ which is an exponential improvement. We aim one step higher to see if we can achieve $O(1)$ worst case shard throughput, the inspiration to achieve this goal is provided by the similarity of equation \ref{eqn:main_function}. 


\paragraph{TP/adv Estimation}
Explain how we estimate Throughput or mining power.

\subsection{\dsab}

We describe \dsab algorithm that ensures that the average throughput of the worst case shard is $h$ where $h$ is a constant. We prove this by showing that the average throughput vector $\boldsymbol{\bar{r}(t)}$ approaches the convex set $C_x$ where $C_x$ denote convex set in $\mathbb{R}^K$ defined as 
\begin{align}
    C_x &= [x,1]^K \quad x \in [0,1] 
\end{align}
we will show that the average throughput vector $\mathbf{\bar{r}}(t)$ converges to $C_{0.5h}$ where $h$ is a constant independent of the number of shards $K$. 

The motivation of the current approach comes from Blackwell approachability theorem which states that if the following conditions hold:
\begin{align}
    \forall \boldsymbol{\beta} \, \exists \boldsymbol{\gamma} \, s.t \, r(\boldsymbol{\gamma},\boldsymbol{\beta}) &\in C_h \label{eqn:blackwell_cond1}\\
    \text{For all half-spaces H containing $C_h$, } &\exists \boldsymbol{\gamma}\, s.t \, \forall\boldsymbol{\beta}\, , r(\boldsymbol{\gamma},\boldsymbol{\beta}) \in H \label{eqn:blackwell_cond2}
\end{align}

then there exists an adaptive strategy $f_t$ such that $\forall \boldsymbol{\beta(1)}, \boldsymbol{\beta(2)}, ..$
\begin{align}
    d\left( \frac{1}{T} \sum_{t=1}^T \boldsymbol{r}(\boldsymbol{\gamma(t)},\boldsymbol{\beta(t)}),C_h \right) \rightarrow 0
\end{align}

where $d$ is the usual euclidean distance metric on $\mathbb{R}^K$ extended to $\mathbb{R}^K \text{X} 2^{\mathbb{R}^K}$ by $d(x,C_h) = \inf_{s\in C_h} d(x,s)$

We observe that condition 1 represented by equation \ref{eqn:blackwell_cond1} is satisfied by setting $\boldsymbol{\gamma} = \frac{\gamma}{\beta}\boldsymbol{\beta}$ and $h=\gamma$. We can also show that condition 2 (equation \ref{eqn:blackwell_cond2}) is satisfied by a honest policy $\boldsymbol{\gamma}$. However, we deviate from the Blackwell approachability result accounting to the stochastic nature of the honest action $\boldsymbol{\Gamma}$ which leads to $\mathbb{E}_{\boldsymbol{\Gamma}}[r_i(t)] \neq \frac{\gamma_i(t)}{\gamma_i(t)+\beta_i(t)}$.

The analysis below will show that even with stochastic allocation $\Gamma_i(t) = \frac{1}{N} \mathit{Binomial}(n,\gamma_i(t))$, $\boldsymbol{\bar{r}(t)}$ approaches $C_h$.

\begin{theorem}
    \dsab algorithm ensures that the throughput of the worst performing shard for an optimal adversary approaches a constant $h$ with the difference diminishing as $O(\sqrt{\frac{K}{T}} + \sqrt[\leftroot{-2}\uproot{2}4]{\frac{1}{T}})$ with finite $N$.
    \label{thm:dsa2}
\end{theorem}

\begin{proof}
    We provide a brief description of the proof below, Please refer to section \ref{sec:proof} for the detailed proof.
    We first prove a \textit{strategy space inequality} which states the following:
    \begin{eqnarray}
     \max_{\mathbf{\gamma}} \min_{\mathbf{\beta}} \sum_{i=1}^{K} u_i \frac{\gamma_i}{\gamma_i+\beta_i} \geq \gamma \frac{s}{K} \sum_{i=1}^{K} u_i \label{eqn:ssi1}
    \end{eqnarray}
    where $u_i = (0.5h-\bar{r}_i)^{+}$, $s = g(N,K)$, the lower bound is achieved by the policy $\tilde{\gamma}_i = \gamma \frac{\tilde{u}_i}{\sum_{i=1}^K \tilde{u}_i}$, where $\tilde{u}_i = u_i$ if $u_i$ is in the highest $s$ in $\boldsymbol{u}$ and 0 otherwise.
    We then modify the target allocation policy as $\boldsymbol{\gamma}$ which ensures that $\gamma_i\geq \frac{b}{K} \forall i \in [K]$ where $b$ is a constant. The new target allocaiton policy can be written as 
    \begin{align}
        \boldsymbol{\gamma} = \frac{1}{1+q/\gamma} \underset{C_{q/s}}{Proj} \, \boldsymbol{\tilde{\gamma}} \label{eqn:blackwell_target}
    \end{align}
    where $\underset{C_{q/s}}{Proj}$ is a projection of the $s$ non-zero values of $\tilde{\gamma}_i$to the set $C_{q/s} = [q/s,1]^s$ and $q = b/(1-2b)$. The new allocation policy leads to a \textit{modified strategy space inequality} given by:
    \begin{align}
        \min_{\boldsymbol{\beta}} \sum_i u_i \frac{\gamma_i}{\gamma_i+\beta_i}  &\geq \frac{s}{K} \gamma(1-2b)   \sum_{i=1}^K u_i
    \end{align}
    We now show that if every honest node chooses a shard randomly according to a choice distribution given by $\boldsymbol{\gamma}$ defined in equation \ref{eqn:blackwell_target}, we get a \textit{stochastic strategy space inequality} given by:
    \begin{align}
        \mathbb{E}_{\boldsymbol{\Gamma(t)}}&\left[\min_{\boldsymbol{\beta(t)}} \boldsymbol{u(t-1)}.\boldsymbol{r(t)} \right] \geq h\sum_{i=1}^K u_i
    \end{align}
    where $h=(1 - s e^{-nc\frac{b}{s}log(c)})c(1-2b)\frac{s}{K}\gamma$.
    We then show that following the above honest allocation strategy yields approaches the convex set $C_h$ with distance decreasing with time $T$ as:
    \begin{align}
         d^2_{T} &\leq \frac{K}{4T} + \frac{2}{T}\sum_{t=1}^{T-1}\frac{t}{T}(Y_t) \label{eqn:blackwell_distance}
    \end{align}
    where  $Y_t = (\mathbb{E}_{\Gamma_i(t)}\left[\sum_i u_i(t-1) r_i(t)\right] - ((\boldsymbol{u(t-1)}).\mathbf{r(t)})$ is a martingale difference sequence w.r.t. history at time $t$ and $|Y_t|\leq 2 h s$, we can now use Azuma- Hoeffding inequality to get:
    \begin{align}
        \mathbb{P}\left( \frac{1}{T} \left\lVert \sum_{t=1}^{T-1} Y_t \right\rVert > \epsilon_m \right) \leq 2 e^{ -\frac{T\epsilon_m^2}{8h^2s^2}} \label{eqn:blackwell_azuma}
    \end{align}
    We can now show that with probability $(1-\delta)$, the distance to convex set converges to 0 as:
    \begin{align}
     d^2_{T} &\leq \frac{K}{4T} + 4hs\sqrt{\frac{2}{T}\log(\frac{2}{\delta})}
\end{align}
\end{proof}

\begin{figure}
    \centering
    \includegraphics[width = .3\textwidth]{images/blackwell1.pdf}
    \caption{Approach to $C_h$}
    \label{fig:blackwell1}
\end{figure}

\textbf{Make comments on N<K and N>K regimes}


\subsubsection{Simulations}
One paragraph to explain simulation
Plots for the minshard TP, made for slides.
Plot for the avg TP shuffling between 2 shards (vector field plot)
Plot with stochastic and keeping the original policy.

Redirect resource usage to section 7.

\begin{figure}
    \centering
    \includegraphics[width = .3\textwidth]{images/latency_bound_adv/avg1.pdf}
    \caption{Adversary N=10K}
    %\label{fig:blackwell1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width = .3\textwidth]{images/latency_bound_adv/avg_zoom1.pdf}
    \caption{Adversary N=10K}
    %\label{fig:blackwell1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width = .3\textwidth]{images/latency_bound_adv/latency1.pdf}
    \caption{Latency: Adversary N=10K}
    %\label{fig:blackwell1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width = .3\textwidth]{images/latency_bound_adv/worst_shard_tp1.pdf}
    \caption{Latency: Adversary N=10K}
    %\label{fig:blackwell1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width = .3\textwidth]{images/latency_bound_adv/avg2.pdf}
    \caption{Adversary N=0.5K}
    %\label{fig:blackwell1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width = .3\textwidth]{images/latency_bound_adv/avg_zoom2.pdf}
    \caption{Adversary N=0.5K}
    %\label{fig:blackwell1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width = .3\textwidth]{images/latency_bound_adv/latency2.pdf}
    \caption{Latency: Adversary N=0.5K}
    %\label{fig:blackwell1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width = .3\textwidth]{images/latency_bound_adv/worst_shard_tp2.pdf}
    \caption{Latency: Adversary N=0.5K}
    %\label{fig:blackwell1}
\end{figure}



==> archive/practical_considerations.tex <==
\subsection{Practical considerations}

{\bf Slow rotation}

==> background.tex <==
\section{Background and Related Work}
\label{sec:relwork}


Blockchain sharding methods in the literature  can be broadly divided into two categories: multiconsensus (most sharding solutions) and uniconsensus architectures. Each of these architectures provide different scaling gains and have distinct security vulnerabilities; we discuss this next. 

\subsection{Multiconsensus architecture}


The multiconsensus architecture relies on each shard having a {\em separate consensus engine} and  allocates nodes randomly to shards  to ensure that each shard has a honest consensus (super)majority. A further periodic random reallocation of nodes to shards protects against a weakly adaptive adversary. The random reallocation is enabled  by a {\em node to shard allocation engine} (N2S) which assigns nodes to shards using a (common) distributed randomness, generated using a  consensus engine shared across all shards and commonly referred to as  {\em beacon consensus engine}. A {\em state commitment engine} posts root of a Merkle Trie \cite{} of a shard's consensus state (the so-called ``state commitment") \cite{} to the beacon consensus engine at regular intervals; this facilitates fast reallocation  and  synchronization to new shards. Figure \ref{fig:n2s1} illustrates these 4 engines and their interactions. 
%Each of the 4 engines   is briefly summarized below. 
\begin{figure}
    \centering
    \includegraphics[width = .48\textwidth]{images/n2s1.pdf}
    \caption{Multiconsensus architecture}
    \label{fig:n2s1}
\end{figure}
%\begin{itemize}
%    \item \textbf{Beacon consensus engine}: Responsible for maintaining a total order log of each shard's state commitment and an allocation of consensus nodes to shards via randomness generated on its log. \textit{Inputs}: Consensus decisions, shard state commitments, node registration. \textit{Outputs}: Total ordered log. \textit{Properties}: Safety, Liveness.
 %   \item \textbf{Shard consensus engine}: Responsible for maintaining total order log of shard transactions.
%    \textit{Inputs}: List of consensus nodes, Consensus decisions, latest state commitment. \textit{Outputs}: Total ordered shard transaction log. \textit{Properties}: Shard safety and liveness.
%    \item \textbf{Node to shard allocation engine}: \textit{Input}: Beacon randomness, node registry. \textit{Output}: Node to shard allocation. \textit{Properties}: N2S allocation ensures honest consensus majority in each shard.
%    \item \textbf{State commitment engine}: \textit{Input}: State commitment, shard votes. \textit{Output}: Post state commitment on beacon consensus engine. \textit{Properties}: State commitments are valid and live.
%\end{itemize}

 {\em Security}. If a (super)majority exists in the overall set of nodes, then the random node to shard allocation engine transfers this property to each shard (as long as each shard is large enough -- this weakness is discussed in detail shortly). This guarantees security of the shard consensus engine, against a static adversary. Periodic reallocation of nodes to shards enhances the security of shard consensus against a slowly adaptive adversary.  

{\em Scaling}. 

Multiconsensus architecture allows nodes to maintain only the state of the shard consensus engine and the beacon consensus engine, with beacon consensus engine only containing state commitments and N2S allocation metadata. Splitting the set of nodes into $K$ different shards, enables parallel execution of $K$ shard consensus engines, thus scaling shard transactions by $O(K)$. It is worth noting that the beacon chain load also increases with $K$ and hence there is an upper bound on the number of shards $K$, that the resource constrained nodes can handle.

Elastico \cite{luu2016secure} and Omniledger \cite{kokoris2018omniledger} pioneered the study and design of sharding methodologies for blockchain in academic literature. Omniledger, built on top of ideas from Elastico, runs N2S allocation using Randhound(a randomization protocol) on an identity blockchain. The nodes are gradually rotated between shards to decrease the synchronization load on the network. Rapidchain \cite{zamani2018rapidchain} further proposed several improvements by reducing the communication complexity to sub-linear in the number of nodes, and secure reallocation of nodes to shards building on the Cuckoo rule. Ethereum Serenity\cite{eth2} uses Casper FFG \cite{buterin2017casper} on the consensus engine to achieve finality and a client focused inter-shard protocol using receipt in state commitments. Polkadot \cite{wood2016polkadot} proposes sharding by splitting roles into 4 parts: Validators, Collators, Fishermen and Nominators and using fraud proofs to improve security.

%Omniledger has a registered validator set on a non sharded beacon blockchain called identity blockchain (beacon consensus engine). Omniledger partitions the validator set by running Randhound (a randomization protocol) on an identity blockchain(N2S allocation engine), the validator subset assigned to each shard changes gradually every epoch. Within an epoch the assigned validator set is responsible for maintaining the shard chain using ByzCoinX which is a voting based BFT consensus protocol(shard consensus engine). The state is checkpointed at the end of each epoch(state commitment engine).

%Ethereum 2.0 \cite{eth2} also involves a central beacon chain(beacon consensus engine) and  multiple  shard  chains(shard consensus engine),  validators  are  rotated  between shards periodically and randomly by the beacon chain(N2S allocation). Beacon chain runs longest chain protocol with Casper FFG finality. A pointer to a shard block is included in the beacon chain as a checkpoint every fixed number of blocks along the shard chain (usually 100). The checkpoint must collect enough votes(majority) to be regarded as a valid latest checkpoint. Each shard chain follows the longest chain rule with the latest checkpoint as genesis.

{\em Vulnerabilities}. The key property enabling security of the multiconsensus architecture is that there is sufficient honest (super)majority in {\em each} shard (this suffices for a static adversary) and the N2S allocation is periodically updated (this allows security against a weakly adaptive adversary). However this comes at the expense of  the following  vulnerabilities:
\begin{enumerate}
    \item \textbf{High number of nodes to shards}: With a random allocation of node to shards, a majority of honest nodes (eg: 75\%) in the total (eg: ) translates to majority of honest nodes in {\em each shard} (eg: number of shards is ) with high probability (eg: ) only if the number of nodes per shard is also large. This restricts the number of shards and thus the scaling capability. 
    \item \textbf{Shard ledger Security}: The N2S allocation is posted on the beacon chain, hence an adversary  knows the list of nodes participating in a target shard. In turn, this situation facilitates the adaptivity of nodes in turning adversarial, thus overstretching beyond the weakly adaptive adversary model and affecting the security.  
 %   \item \textbf{Identity maintenance}: The  nodes need to make their blockchain identity public which is fine for permissioned blockchain, but a deviation from Bitcoin like permissionless blockchains.
\end{enumerate}

%These sharding protocols justify the safety and liveness attack by assuming that the adaptive adversary is slower that the periodic rate at which N2S allocation is called which is very powerful assumption since adversaries can typically be assumed faster than honest nodes.
Ethereum 2.0 \cite{eth2} and Polkadot \cite{wood2016polkadot} attempt to extend the range of adaptive adversaries they can safely handle by  introducing state transition validity fraud proofs \cite{teutsch2019scalable} for state commitments; however, this does not solve the liveness vulnerability and does not solve the safety vulnerability {\em between} state commitments. In general, security of sharding against adaptive adversaries remains a major challenge; addressing this is the main focus of the uniconsensus architecture discussed next. 


\subsection{Uniconsensus architecture}
\label{sec:uniconsensus}
\begin{figure}
    \centering
    \includegraphics[width = .4\textwidth]{images/trivial_sa.pdf}
    \caption{Uniconsensus architecture}
    \label{fig:trivial_sa}
\end{figure}

The uniconsensus architecture relies on a single {\em consensus engine} to maintain {\em all} shards, thus the safety of each shard can be directly derived from the safety of the main consensus engine. The consensus engine only maintains a {\em log of hash of shard blocks} and hence is scalable. A honest consensus (super)majority is no longer needed in each shard, thus each node is free to join a shard of it's choice (self-allocation) and run a {\em shard log maintainer} responsible for validating and mining shard blocks. Shard block validation is performed by shard nodes and is decoupled from shard block ordering performed by the consensus engine. The consensus engine only gets the hash of a shard block which may be mined by an adversary which does not publish the full block;  such a data withholding can lead to a fatal liveness attack and is averted by recourse to a {\em data availability engine}.  Figure \ref{fig:trivial_sa} illustrates the 3 engines and their interactions. 
%Each of the 3 engines are briefly summarized below.
%\begin{itemize}
%    \item \textbf{Consensus engine}: Responsible for maintaining a log of all shard block accumulators. \textit{Input}: Shard block pointers, shard block mining proof, shard block availability proof. \textit{Output}: Total ordered log of shard block pointers. \textit{Properties}: Safety and liveness
%    \item \textbf{Shard log maintainer}: Responsible for mining shard blocks and maintaining consensus-validity decoupled shard ledger. \textit{Input}: (Shard transactions, mining oracle), (Total ordered log, shard blocks). \textit{Output}: (Shard block), (Sanitized shard ledger).\textit{Properties}: Shard blocks pointed by consensus engine are available.
%    \item \textbf{Data availability engine}: \textit{Input}: Check availability of a shard block. \textit{Output}: Availability of shard block. \textit{Properties}: Compute and storage $O(1)$ in the number of shards $K$. 
%\end{itemize}

{\em Security:} If a consensus (super)majority exists in the overall set of nodes, the consensus engine is secure. Consider a shard with less than a majority of honest nodes, the adversarial nodes in the shard cannot change the log of shard blocks without violating safety of the consensus engine, thus an adaptive adversary with less than a global consensus majority cannot violate safety of any shard. The lack of honest majority constraint within a shard also allows for small shard size. We observe that uniconsensus architecture solves the shard ledger safety and shard size vulnerabilities of multiconsensus architecture, but introduces new liveness vulnerabilities discussed below. 

{\em Scaling:} Nodes maintaining the uniconsensus architecture only maintain the consensus engine and shard log of one shard, the consensus engine contains a log of shard block hashes, the size of which is much smaller than shard blocks. Thus, $K$ shards can be processed in parallel with each node processing only one shard log. Note that similar to multiconsensus architecture, the load on the consensus engine increases with the number of shards, hence $K$ is upper bounded by the throughput of the consensus engine.

Distributed systems architectures like Corfu \cite{balakrishnan2012corfu} used a single shard log (similar to consensus engine) to organize a cluster of flash drives and Tango \cite{balakrishnan2013tango} to provide an interface with the scaled databases log(Corfu) that scales to the limit of the underlying log. Blockchain protocols like Mastercoin \cite{} and Lazyledger \cite{lazyledger} also scale using uniconsensus by using a central blockchain like bitcoin to commit accumulators of their transactions. Other partial scaling works like Aspen \cite{gencer2017short} and SSChain \cite{chen2019sschain} also adopt the uniconsensus architecture.
%The idea of uniconsensus architecture was proposed in an early practical work, Mastercoin \cite{}, which was proposed in 2012, as a practical way of scaling at  bitcoin-level security.  The key idea is to write Mastercoin transactions in the unparsed fields of Bitcoin transactions. Since Bitcoin nodes are unaware of Mastercoin, they do not check the validity of these transactions. The Mastercoin nodes then sanitize these transactions in the order that they appear in the Bitcoin ledger, thus providing high security. Furthermore, Mastercoin does not impose any computational burden on the Bitcoin network, although it does impose  storage and communication burden on the Bitcoin ledger. This idea is explored in a recent work LazyLedger \cite{lazyledger}, which scales  the communication complexity using data availability proofs  \cite{al2018fraud}. Other partial scaling works like Aspen \cite{gencer2017short} and SSChain \cite{chen2019sschain} also adopt the uniconsensus architecture.


{\em Vulnerability:} Removing N2S allocation by allowing node self-allocation introduces a liveness attack on a shard where an adversary can concentrate it's mining power on one shard and drown out honest shard blocks; in this attack, the fraction of honest blocks to the adversarial blocks is greatly reduced due to a large fraction of adversarial nodes in the shard. Since the shard has limited resources, it can only support a fixed number of shard blocks, hence a low honest block to total block fraction would lead to a throttling of the number of honest shard blocks added to the shard log and hence throttle throughput. The honest transactions can no longer be processed in finite time, thus leading to loss of liveness. An example of this attack is shown in figure \ref{fig:tp_suppression}.  
A proposed solution \cite{} to reducing this vulnerability is to allow only a permissioned set shard nodes to mine shard blocks, which is not secure since the adaptive adversary knows the static set of such permssioned nodes. In general, liveness in the uniconsensus architecture against adaptive adversary is a major security challenge. 

To summarize: the multiconsensus sharding architecture's safety is vulnerable to adaptive adversaries and the uniconsensus sharding architecture's liveness is vulnerable  to adaptive adversaries. 

\subsection{Overview of \tfp}
\label{sec:overview}

The main contribution of this paper is the introduction of the \tfp architecture which provides full horizontal scaling (in all the 3 dimensions of storage, compute and communication) while being secure against fully adaptive adversaries. The architecture, depicted in Figure~\ref{fig:overview} is a combination of the building blocks from {\em both} multiconsensus and  uniconsensus architectures, {\em glued together} with a new engine: the {\em dynamic self-allocation (DSA) engine}. The dynamic self-allocation engine provides an algorithm for honest nodes to re-allocate themselves to shards, thus reacting to adversaries congregating in individual shards, and guarantees a strong mathematical property: the {\em time average} fraction of honest to adversarial nodes in every shard is greater than any desired constant fraction.  
Deriving this dynamic self-allocation engine and its mathematical guarantee is a core algorithmic and theoretical contribution of this paper and is discussed in detail in the next section. 

The \tfp architecture shares the consensus engine, shard log maintainer and data availability engines with the uniconsensus architecture. Shard log is derived from the consensus engine and maintained by shard nodes. The shard nodes change their allocation dynamically by calling the DSA engine locally at regular time intervals. The nodes synchronize to the newly allocated shard using the state commitments from the state commitment engine which works in a similar manner as its counterpart in multiconsensus architecture. Figure \ref{fig:overview} illustrates the 5 engines and their interactions.

\begin{figure}
    \centering
    \includegraphics[width = .48\textwidth]{images/overview1.pdf}
    \caption{Trifecta Architecture}
    \label{fig:overview}
\end{figure}

We provide a short summary of the main security and scalability properties of \tfp below. A formal statement and proof of these properties is deferred to Section~\ref{}. 

{\em Security}: Small shard size and shard safety properties can be derived from the uniconsensus architecture. The DSA engine ensures that the time average fraction of honest to adversarial nodes in every shard is greater than any desired constant fraction. Thus, adversaries cannot follow a strategy where they can cause a liveness attack by reducing the fraction of honest to adversarial nodes.

{\em Scalability:} Consensus engine is scalable since only shard block hash and state commitments (Merkle roots) are ordered using the consensus engine. Since the time average fraction of honest nodes to adversarial nodes in a shard is greater than a desired fraction, so is the ratio of honest blocks to the adversarial blocks. Since a shard node can maintain shard blocks at a constant rate, a fraction of which is constant, it can achieve $O(1)$ throughput per shard, with $K$ shards, the total throughput is $O(K)$. Resource usage for synchronizing to a new shard is reduced  by reducing the time interval between state commitments. 



\subsection{Our Contribution}
\subsubsection{Model} 

Consider a network with $N$ nodes. While our architecture and results are applicable more generally, we will assume a homogeneous network where all nodes have the same amount of resources. We will particularly be concerned about three types of resources: (1) computation resource - the number of transactions executed per second, (2) storage resource - the number of transactions / second that can be incrementally stored by the node \footnote{We will make the simplifying assumption that the storage per node is growing with time. This is required for Bitcoin for example. Ideas to relax this requirement, for example \cite{MimbleWimble}, can be naturally applied to our setting too.} and (3) communication resource - the bandwidth of data exchanged by the node. We will assume that at every node, {\bf all three resources are sufficient} to run a non-sharded blockchain with $R$ transactions-per-second. We will assume that, at any given time, a fraction $\beta$ of nodes are controlled  by the adversary - they can deviate arbitrarily from the proposed protocol. We will allow a {\em fully adaptive adversary}, which can corrupt any node based on the public state. We will assume that the underlying communication network is synchronous, even though our protocol can be extended to asynchronous settings as well.  


{\bf Key Properties} \tfp satisfies the following properties: 
\begin{itemize}
    \item \tfp is safe as long as $\beta < 0.5$ fraction of nodes are controlled by the adversary.
    \item \tfp is live as long as $\gamma > 0$ fraction of nodes follow the self-allocation policy. 
    \item \tfp can support $K < \Theta(\frac{N} {\log N})$ shards each of throughput at least $R/2$ transactions per second. Thus we get a total scaling of $\Theta(\frac{N} {\log N})$ relative to running a single shard.
\end{itemize}





{We require the remaining $1-\beta$ honest nodes to follow the underlying consensus protocol but they need not comply with the self-allocation policy.}

We require three key primitives from previous literature in order to achieve the aforementioned properties. 
 {\bf State Machine Replication} A totally ordered log of the shard block headers is maintained using a SMR \cite{SMR}. We assume that the SMR is robust to an adversary adaptively corrupting at most $\beta_{c}$ fraction of the nodes. To achieve scalability, we require that the total message complexity of SMR be linear in the number of nodes (so that the complexity per node is a constant).  
 
 Examples of SMR that satisfy these properties include Ouroboros Praos and Algorand, since they are robust to fully adaptive adversaries. We note that Ouroboros Praos has $\beta_c = 0.5$ whereas Algorand has $\beta_c=\frac{1}{3}$. Other protocols which have efficient communication complexity such as HotStuff \cite{}, Sync HotStuff \cite{}, and Streamlet \cite{} are robust to varying degrees of adaptivity. 

 {\bf Data Availability engine}: We require data availability engine as a key primitive.  \textit{Input}: Commitment $c$ for a shard block (of size $B$) from a honest / adversarial node. \textit{Output}: Every node deduces correctly if the block is available. 
 \textit{Properties}:  Nodes inside that shard expend at most $O(B \log B)$ resources. Every node expends at most $O(\log B)$ resources.
  \textit{Assumption}: Correct if at least one honest node inside the shard.

    
\textbf{State commitment engine}: \textit{Input}: Previous state commitment $c$, block $B$ of transactions, claimed state $s$ after executing $B$ beyond $c$. \textit{Output}: Every node correctly agrees on whether $s$ is correct or not. 
\textit{Properties}: Requires a distinct committee for $R = O(\log B)$ rounds. Every committee member spends at most $O(B \log B)$ resources. All other nodes expend at most $O(\log B)$ resources. 
 \textit{Assumption}: Correct if at least one honest node in the committee of each round.


    

==> bg_overview.tex <==
1. Multiconsensus
-> Separate SMR for each shard
-> Post periodic commitments into a common shard 

Node-to-shard allocation done through the common SMR engine. 

Safe against Weakly adaptive adversaries

Adaptive Adversary
a) Safety violation: 

b) Liveness violation


Cryptographic methods such as ZK-STARK and verifiable computing  still have liveness violation

2. Uniconsensus
Decoupled consensus common in BFT methods
Corfu created a shared log in a distributed system  and Tango created a sharded application system on top of hte distriobuted log. 

Lazyledger has proposed such a similar architecture recently. Not for sharding.

Vulnerability

What picture to use? 

Trifecta 

==> commands.tex <==
% !TEX root =  main.tex

\usepackage{comment}
\usepackage{graphicx,subcaption}
\usepackage{varwidth}
\usepackage{authblk}

\setcounter{secnumdepth}{3} % numbering section depth
\setcounter{tocdepth}{4}

\newtheorem{thm}{Theorem}[section]
\newtheorem{defn}[thm]{Definition}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{prop}{Proposition}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{constr}[thm]{Construction}


\newcommand{\bpf}{\begin{proof}}
\newcommand{\epf}{\end{proof}}
\newcommand{\bprf}{{\em Proof: }}
\newcommand{\bproof}{{\em Proof of }}
\newcommand{\eproof}{\hfill $\Box$}
\newcommand{\argmin}{\operatornamewithlimits{arg \ min}}
\newcommand{\argmax}{\operatornamewithlimits{arg \ max}}
\newcommand{\indep}{\mathrel{\text{\scalebox{1.07}{$\perp\mkern-10mu\perp$}}}}


%\newcommand{\red}[1]{\textcolor{red}{#1}}
%\newcommand{\blue}[1]{{#1}}

\newcommand{\beqa}{\begin{eqnarray}}

\newcommand{\eeqa}{\end{eqnarray}}

\newcommand{\beqan}{\begin{eqnarray*}}

\newcommand{\eeqan}{\end{eqnarray*}}

\newcommand{\beq}{\begin{equation}}

\newcommand{\eeq}{\end{equation}}

\newcommand{\prf}{\noindent {\bf Proof}\ \ \ }

\newcommand{\lra}{\Longleftrightarrow}

\newcommand{\lbr}{\left \{ }

\newcommand{\rbr}{\right \} }

\newcommand{\Lbr}{\left [}

\newcommand{\Rbr}{\right ]}

\newcommand{\lp}{\left (}

\newcommand{\rp}{\right )}

\renewcommand{\r}{\right}

\renewcommand{\l}{\left}

\newcommand{\df}{\stackrel{{\rm def}}{=}}

\newcommand{\real}{{\Bbb {R}}}

\newcommand{\complex}{{\Bbb {C}}}

\newcommand{\prob}{{\Bbb {P}}}

\newcommand{\expect}{{E}}

% \newcommand{\eqref}[1]{(\ref{#1})}




\newcommand{\X}{{\mathcal X}}

\renewcommand{\S}{{\cal S}}

\newcommand{\bmk}{\beta_m^{(K)}}



\newcommand{\vu}{{\bf u}}

\newcommand{\vd}{{\bf d}}

\newcommand{\Ummse}{U_{{\rm mmse}}}

\newcommand{\vp}{{\bf p}}

\newcommand{\vq}{{\bf q}}

\newcommand{\vone}{{\bf 1}}

\newcommand{\vh}{{\bf h}}
\newcommand{\hh}{\hat h}
\newcommand{\vw}{{\bf w}}

\newcommand{\SNR}{\sf SNR}
\newcommand{\SINR}{\sf SINR}
\newcommand{\rot}{\sf RoT}
\newcommand{\penal}{\sf penalty}
\newcommand{\PR}{\sf PR}

\newcommand{\eapprox} {\stackrel {.}{=}}
\newcommand{\al}{\stackrel{.}{<}}
\newcommand{\ag}{\stackrel{.}{>}}

\newcommand{\SINRt}{{\sf SINR^{(t)}}}
\newcommand{\lambdat}{\lambda^{(t)}}
\newcommand{\It}{I^{(t)}}
\newcommand{\vwt}{{\bf w}^{(t)}}
\newcommand{\vwn}{{\bf w}^{(t+1)}}
\newcommand{\vv}{{\bf v}}
\newcommand{\uu}{{\bf u}}
\newcommand{\ww}{{\bf w}}
\newcommand{\eps}{\varepsilon}
\newcommand{\vz}{{\bf z}}
\newcommand{\bvh}{\bar{\vh}}



\newcommand{\singlespacing}{\let\CS=\@currsize\renewcommand{\baselinestretch}{0.95}\tiny\CS}



\newcommand{\oneandahalfspacing}{\let\CS=\@currsize\renewcommand{\baselinestretch}{1.25}\tiny\CS}



\newcommand{\doublespacing}{\let\CS=\@currsize\renewcommand{\baselinestretch}{1.39}\tiny\CS}



% Start with double spacing:

%%\singlespacing

%\oneandahalfspacing

%\doublespacing

\newcommand{\be}{\begin{equation}}

\newcommand{\ee}{\end{equation}}

\newcommand{\tr}{{\rm trace}}

\newcommand{\rref}[1]{(\ref{#1})}

\newcommand{\CN}{{\cal CN}}





\newcommand{\bc}{\begin{center}}

\newcommand{\ec}{\end{center}}

\newcommand{\bfl}{\begin{flushleft}}

\newcommand{\efl}{\end{flushleft}}

\newcommand{\blob}{\hfill \rule{.1in}{0.1in}}
\newcommand{\prism}{{\sf Prism }}
\newcommand{\tf}{{\sf Trifecta }}
\newcommand{\tfnosp}{{\sf Trifecta}\ignorespaces}
\newcommand{\scheme}{{\sf Prism} }
\newcommand{\schemenosp}{{\sf Prism}\ignorespaces}
\newcommand{\schemelite}{{\sf Prism 1.0 } }
\newcommand{\schemelitenosp}{{\sf Prism 1.0}\ignorespaces}
\newcommand{\schemebackbone}{{\sf Prism Backbone} }
\newcommand{\schemebackbonenosp}{{\sf Prism Backbone}\ignorespaces}
\newcommand{\fruitchains}{{\sf Fruitchains } }
\newcommand{\fruitchainsnosp}{{\sf Fruitchains}\ignorespaces}
\newcommand{\bitcoinNG}{{\sf BitcoinNG } }
\newcommand{\bitcoinNGnosp}{{\sf BitcoinNG}\ignorespaces}
\newcommand{\disccoin}{{\sf DiscCoin } }
\newcommand{\disccoinnosp}{{\sf DiscCoin}\ignorespaces}
\newcommand{\byzcoin}{{\sf ByzCoin } }
\newcommand{\byzcoinnosp}{{\sf ByzCoin}\ignorespaces}
\newcommand{\hybrid}{{\sf Hybrid } }
\newcommand{\thunderella}{{\sf Thunderella }}
\newcommand{\inclusive}{{\sf Inclusive }}
\newcommand{\spectre}{{\sf Spectre }}
\renewcommand{\phantom}{{\sf Phantom }}
\newcommand{\conflux}{{\sf Conflux }}
\newcommand{\avalanche}{{\sf Avalanche }}
%%\newcommamd{\rust}{{\sf Rust}}
\newcommand{\bitcoin}{{\sf Bitcoin} }
\newcommand{\bitcoinnosp}{{\sf Bitcoin}\ignorespaces}

\newcommand{\ghost}{{\sf GHOST} }
\newcommand{\ghostnosp}{{\sf GHOST}\ignorespaces}

\newcommand{\pois}{{\sf Poiss}}
\newcommand{\geom}{{\sf Geometric}}
\newcommand{\bin}{{\sf Bin}}

\makeatletter
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                       {-18\p@ \@plus -4\p@ \@minus -4\p@}%
                       {4\p@ \@plus 2\p@ \@minus 2\p@}%
                       {\normalfont\normalsize\bfseries\boldmath
                        \rightskip=\z@ \@plus 8em\pretolerance=10000 }}

\newcommand{\ext}{{\sf ext} }

\newcommand{\N}{{\mathcal{N}}}
\newcommand{\Z}{{\mathcal{Z}}}
\newcommand{\fv}{\bar{f}_v}
\newcommand{\fp}{\bar{f}_p}
\newcommand{\Rl}{R_{\ell}}



\newcommand{\Vo}{{\sf{V}}}
\renewcommand{\H}{{\mathcal{H}}}
\newcommand{\C}{{\mathcal{C}}}
\newcommand{\Q}{{\mathcal{Q}}}
\newcommand{\A}{{\mathcal{A}}}
\newcommand{\T}{{\mathcal{T}}}
\newcommand{\R}{{\mathcal{R}}}
\newcommand{\rmax}{r_{\rm max}}
\newcommand{\rmin}{r_{\rm min}}
\newcommand{\bmin}{b_{\rm min}}
\newcommand{\kmin}{k_{\rm min}}
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\P}{{\mathcal P}}
\newcommand{\Dr}{{\Delta_r}}
\newcommand{\Dmax}{{\Delta_{\text{max}}}}
\newcommand{\cone}{\frac{1-2\beta}{16}}


\makeatother
\newcommand{\blue}{\color{blue}}

\newcommand{\tE}{\texttt{E}}
\newcommand{\tT}{\texttt{T}}
\newcommand{\tF}{\texttt{F}}
\newcommand{\Rc}{R^{\text{stop}}}
\newcommand{\Rconf}{R^{\text{conf}}}
\newcommand{\Dll}{D_{\ell', \ell}}
\newcommand{\Dllf}{\big\{D_{\ell', \ell}\big\}_{\ell'\leq \ell}}
\newcommand{\Rfirst}{R_0}
\newcommand{\Rlast}{R_{\text{last}}}
\newcommand{\LS}{\texttt{LedSeq}}
\renewcommand{\epsilon}{\varepsilon}

\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{xcolor}
\definecolor{azure}{rgb}{0.54, 0.17, 0.89}
\newcommand{\colorcomment}[1]{\Comment{ {\color{azure} #1}} }
\newcommand{\av}[1]{$#1$}
\newcommand{\maincolorcomment}[1]{{\color{azure}// #1 } }
\def\NoNumberLine#1{{\def\alglinenumber##1{}\State #1}\addtocounter{ALG@line}{-1}}
\usepackage{enumitem,kantlipsum}

\newcommand{\dt}[1] {{\textcolor{green}{DT: #1}}}
\newcommand{\rr}[1] {{\textcolor{cyan}{RR: #1}}}
\newcommand{\pv}[1] {{\textcolor{purple}{PV: #1}}}


\renewcommand{\bmin}{B_{\rm min}}
\newcommand{\tflc}{{\sf Trifecta Longest Chain} }
\newcommand{\tflcnosp}{{\sf Trifecta Longest Chain}\ignorespaces}
\newcommand{\proposer}{{proposer} }
\newcommand{\Proposer}{{Proposer} }

\usepackage{mathtools}
\usepackage{amssymb}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\usepackage{hyperref}
\newcommand{\calM}{{\mathcal M}}

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
Altruistic minority can stabilize a corruptible majority.




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:




==> efficiency.tex <==
\section{Efficiency}

Model definition (similar to trifecta)
Resource model highlighting limited resource.
Resource usage calculation
Showing O(1) resource usage
Give efficiency theorem (stating limited usage)


==> general.tex <==
\section{General protocol}
\label{sec:general}

Our sharding protocol relies on a central consensus engine maintained by all the peers in the network to create a totally ordered log of blocks and state commitments of all shards. This central consensus engine is responsible for safety of each shard. Moreover, each peer can join any shard it wants and mine blocks on it, doing so in a naive way however runs us at a risk of an adversary mining shard blocks on one shard and throttling a shard's throughput thus hurting liveness. We propose a self-allocation algorithm that manages any king of adversarial throttling attack and ensures a O(1) throughput in each shard. We explain this protocol is more detail below.

\subsection{Consensus Engine}
All peers maintain a central consensus engine. This consensus engine is responsible for maintaining a Total ordered log of the following entries:
\begin{itemize}
    \item \textbf{Shard block pointers:} Shard block pointers are merely a tuple (shard id, hash of a shard block). A total ordered log of these shard pointers can be used to create a shard ledger.
    \item \textbf{Shard state commitment:} State root of a Merkle Patricia tree formed by a version of the state of a shard. It is maintained in the form of a tuple (State root, shard id, version), where the version is the index at which the state commitment was taken.
    \item \textbf{Peer registry:} The peer registry is maintained for the consensus engine, and can be ignored if the consensus engine is identity-less like PoW. It is important to note that the peer registry does not maintain the shard maintained by the registered peer, this is done to ensure that it's difficult for an adaptive adversary know the peers maintaining it's target shard.
\end{itemize}

The total ordered log can be created by a consensus engine running any any consensus algorithm ranging from Atomic broadcast to voting based BFT to even permissionless Nakamoto PoW. The maintainers of the consensus engine need to do the following checks before adding an entry to the total ordered log:
\begin{itemize}
    \item \textbf{Shard block data validity:} Peers need to ensure that the shard block pointers are pointing to a shard block which is available to honest peers. This can be naively done downloading complete shard blocks of all shards at the cost of a huge communication burden. We instead ensure this by using a Coded Merkle Tree construction which ensures O(1) communication load even with $K$ shards.
    \item \textbf{Shard block mining validity:} Peers need to ensure that the shard blocks pointed to are mined correctly, this can be done by check the mining proof corresponding to a shard block pointer.
    \item \textbf{Shard state commitment validity:} We need to ensure that the state commitments are valid, i.e. it corresponds to a valid state transition function applied to that shard's ledger. To ensure that peers maintaining the consensus engine do not have to perform state transition on each shard's ledger, we use a state commitment engine.
\end{itemize}

Note that the checks mentioned above do not require peers to download and perform State transition on shard blocks, thus scaling down the computation, communication and storage load on the peers to maintain the consensus engine.

\subsection{Shard maintainer}
A peer allocates itself to a shard and maintains it. Shard maintenance broadly consists of 3 tasks as mentioned below:
\begin{itemize}
    \item \textbf{Shard ledger maintenance:} The peer downloads all blocks pertaining to its shard (shard id $i$) and orders them according to the total order log. The peer goes through the total order log and filters shard pointers with shard id $i$. The shard blocks are ordered according to the filtered pointers and these ordered shard blocks create a shard ledger
    \item \textbf{Shard ledger sanitization:} The shard ledger created above may contain invalid transactions, this happens because the consensus engine does not check the validity of transactions(since it does not download and process shard blocks), hence it may include shard blocks that contain invalid transactions. The sanitization works by traversing the shard ledger from genesis and ignoring any invalid transaction, the peer may additionally store a validity bit-mask locally to restore the results of the sanitization. Notice that all peers maintaining the shard have consensus on the ordering of the shard ledger and hence will produce the same validity bit-mask after sanitization. This decoupling of consensus and validity is essential is ensuring that safety is maintained by the consensus majority of nodes in the network while simultaneously lowering resource load on consensus peers due to all shard ledgers.
    \item \textbf{Shard block mining:} The peer maintains a list of shard transactions that are not yet included in the shard ledger and creates a shard block containing them. The shard block does not have a pointer to a previous shard block as shard blocks are not responsible for ordering. Once a shard block is created, the peer mines the block to be included in the totally ordered log. The mining process is pluggable and can range from PoW based mining with $Hash(shard block,\, nonce) < shardThreshold$ or can involve permissioned mining using VRF as follows: $VRFEvaluate(peer_Skey,\, latest\, TotalOrderLogBlockHash) < shardThreshold$(This will not work). In the permissioned setting, an accumulator of the shard block needs to be signed by the peer to check mining validity.
    (DOUBT: Do i mention fruitchain hooks here)
    \item \textbf{Shard state commitment:} The peer posts state commitment on the total ordered log by using the state commitment engine.
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width = .48\textwidth]{images/shard_log.pdf}
    \caption{Shard log maintainer}
    \label{fig:shard_log}
\end{figure}



\subsection{Dynamic self allocation engine}
Explain dynamic self allocation engine. Each node picks a shard based on the previous inputs.
PROBLEM: HOW much do we discuss our policy.
Say that we have an algorithm that ensures min TP of 1/2. \\
Let $\gamma_i(t)$ and $\beta_i(t)$ denote the normalized honest and adversarial shard block mining power for shard $i$ at time $t$. All the mined shard blocks are eventually ordered by the consensus engine, thus the fraction of honest shard $i$ blocks in the total ordered log is $\frac{\gamma_i(t)}{\gamma_i(t)+\beta_i(t)}$, we adjust a shard's mining threshold to ensure that the total number of shard $i$ blocks mined per unit time stays constant. Hence the throughput for shard $i$ at time $t$ is given by $\frac{\gamma_i(t)}{\gamma_i(t)+\beta_i(t)}$ considering the worst thing an adversary can do to throttle throughput is to mine empty shard blocks. Let $\gamma$ and $\beta$ denote the normalized total honest mining power and adversarial mining power respectively with $\gamma+\beta=1$.\\
Consider a system with K shards and a naive honest strategy of allocating uniformly to all shards, thus ensuring $\gamma_i(t) = \frac{\gamma}{K}$. The adversary, being free to choose its own shard can concentrate on shard $i$, thus $\beta_i(t)=\beta$, thus throttling the throughput of that shard to $\frac{\gamma/K}{\gamma/K + \beta} = O(1/K)$. This is a fatal attack on the liveness of shard $i$ since honest transactions in that shard can barely be published. We introduce a novel dynamic self-allocation algorithm that can be followed by the honest nodes to ensure that the time averaged throughput of every shard is greater than $h$ where $h$ is a back-off factor independent of $K$. The dynamic self-allocation is handled by the DSA engine with black-box functionality described as follows:
\begin{enumerate}
    \item \textbf{Suggest allocation:} This functionality provides a suggested shard which a peer should maintain in the next time step (DOUBT: define time step). If a constant factor of honest peers follow this suggestion, we can ensure that the time averaged throughput of every shard is greater than a constant $h$. This functionality has the following i/o:
    \begin{itemize}
        \item \textit{Input:} Total ordered log, lower estimate of the factor of honest peers following the protocol
        \item \textit{Output:} Suggested shard to maintain.
    \end{itemize}
    \item \textbf{Allocated shard synchronization:} Not sure to put it here or in state commitment.
\end{enumerate}




\subsection{State commitment engine}
Discuss that we need to sync to new shard as can't maintain ledger of each shard\\
When allocating to a new shard, use latest state commitment + ledger after state commitment.

We divide timeline on the consensus ordered log into epochs where miners on each shard post commitment of the state root at the end of an epoch. This state commitment can be used for a variety of purposes like synchronizing to a newly self-allocated shard or processing inter-shard transaction from another shard.

The state commitment module provides the following functionalities:
\begin{enumerate}
    \item \textbf{Get committee membership:} Be part of the shard committee which enables a peer to post and challenge(optional) state commitment. A shard committee is reevaluated after a fixed number of epochs through any mining mechanism of the designer's choice. This functionality has the following i/o
    \begin{itemize}
        \item \textit{Input:} Committee membership mining, shard id, epoch number
        \item \textit{Output:} Committee membership proof.
    \end{itemize}
    
    \item \textbf{Latest state commitment:} Provides the state root for a shard $i$, which is the latest state root committed according to the order of the consensus engine. The state root is a root of an ordered Merkle Patricia tree of the state. It has the following i/o
    \begin{itemize}
        \item \textit{Input:} Consensus ordered log, shard id: $i$
        \item \textit{Output:} Latest valid state root for shard $i$
    \end{itemize}
    \item \textbf{Submit state commitment:} Publish the latest state commitment for shard $i$ to be ordered on the consensus ordered log. The state commitment is only accepted by peers participating in the consensus engine if the commitment is valid. This functionality has the following i/o.
    \begin{itemize}
        \item \textit{Input:} State root, consensus ordered log index at which the state snapshot was taken, shard id, committee membership proof
        \item{Output:} Consensus on validity of state root
    \end{itemize}
    \item \textbf{Challenge state commitment(optional):} Submit a challenge to a circulated state commitment if it's invalid. This process is interactive and involves an interactive approach to narrow down the challenges. This functionality has the following i/o:
    \begin{itemize}
        \item \textit{Input:} State commitment being challenged, proof of invalidity of state commitment, committee membership proof
        \item \textit{Output:} Challenge validity 
    \end{itemize}
\end{enumerate}

\subsection{Data availability engine}
Every peer maintaining the consensus engine needs to make sure that the shard block pointers in the total order log point to a shard block which is available to all honest nodes. This is trivially ensured by the downloading blocks from all shards to ensure data availability. The naive approach however, is prohibitively expensive in communication for a large number of shards. We propose using erasure coding based approach to ensure Data availability by using CMT. The Data availability engine ensures the following 2 properties:
\begin{itemize}
    \item \textbf{Soundness:} If a peer maintaining consensus engine has concluded that a shard block for shard $i$ is fully available, then at least one honest peer in shard $i$ will be able to fully recover this block within a constant delay of $\Delta_c$.
    \item \textbf{Agreement:} If a peer maintaining consensus engine has concluded that a shard block for shard $i$ is fully available, then all the other peers maintaining the consensus engine will conclude that the block is fully available within a constant delay of $\Delta_c$.
\end{itemize}
The module has the following functionalities:
\begin{enumerate}
    \item \textbf{Check availability:} This functionality checks if the data of a shard block is available and returns a unavailablity proof of constant size if data is not available. The cost of participating in this functionality is also constant with increasing number of shards. This functionality has the following i/o:
    \begin{itemize}
        \item \textit{input:} Shard block hash, CMT root
        \item \textit{output:} Availability status, Unavailability proof
    \end{itemize}
    \item \textbf{Store samples:} This functionality stores random leaf samples of a shards CMT. These samples along with the ones stored by other peers can be used to prove data invalidity.This functionality has the following i/o:
    \begin{itemize}
        \item \textit{input:} Shard block hash, CMT root, random CMT leafs
        \item \textit{output:} None
    \end{itemize}
\end{enumerate}

\subsection{Main theorem}
Safety

\subsubsection{Safety intuition}
Shard security comes from consensus engine.
Give example of a 1 honest miner shard.


Liveness through throughput bounds


==> images/mainflow.tex <==
% \section{Diagrammatic view of Multisketch operations}\label{app:mainflow}  

% A user registers with a user id $\u$ and a vector of biometric templates
% $\mvec=\mvecss{\mlen}$. Multisketch uses two databases $\dbid$ and $\dbmsg$\@,
% where $\dbid$ contains user id $\u$ and the corresponding helper data
% $\sketchval$, and $\dbmsg$ contains the random permutation of the templates
% registered so far. Highlighted are the entries corresponding to a user $\u_4$
% with templates $\mvec_4=\mvec_{41}\ldots\mvec_{4\mlen}$.% and helper
%     % data $\sketchval_4$.
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[
    >=stealth,
    node distance=2cm,
    database/.style={
      cylinder,
      cylinder uses custom fill,
      cylinder body fill=black!25!white,
      cylinder end fill=black!25!white,
      shape border rotate=90,
      aspect=0.25,
      minimum width=2em,
      minimum height=2em,
      draw
    },
    func/.style={
      rectangle,
      fill=red!25!white,
      minimum width=1cm,
      minimum height=1em,
      draw
    },
    cell/.style={
      rectangle,
      draw=black!50!white
    }
    ]
    \node (user) at (0, 0) {User};
    \node[func, right of=user, right=-1.1em, above=3em] (msketch) {$\MS$}; 
    \draw[below of=msketch, dashed, anchor=west] (.85,0.55) rectangle (5.9,-1.2); 
    \node[func, below of=msketch, anchor=east, below=1.95cm,fill=red!10!white,dashed] (mrecover) {$\MRec$};
    % \node[database, right of=user, anchor=south, above=1em, right=2cm] (db1) {$\dbid$};
    \matrix (db1) [right of=user, anchor=south, below=2pt, right=-0.1cm, 
    matrix of math nodes,
    column sep = -\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}}, 
    column 2/.style={nodes={cell}}, 
    anchor=west] {
      \u_1 & \sketchval_1\\
      \u_2 & \sketchval_2\\
      \u_3 & \sketchval_3\\
      |[draw,fill=blue!20]|\u_4 & |[draw,fill=blue!20]|\sketchval_4\\
    };
    \node[left of=db1, anchor=east,right=1.1cm] {$\dbid$};
    \matrix (db2) [right of=db1, left=25pt, matrix of math nodes,
    column sep = 2\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}},
    column 2/.style={nodes={cell}}, 
    column 3/.style={nodes={cell}}, 
    column 4/.style={nodes={cell}}, 
    column 5/.style={nodes={cell}}, 
    anchor=west] {
      \mvec_{21} &\mvec_{12} & |[draw,fill=blue!20]|\mvec_{43} &  & \mvec_{3\mlen} \\
      |[draw,fill=blue!20]|\mvec_{41} &\mvec_{32} & \mvec_{33} & |[draw=white]|\ldots & \mvec_{2\mlen} \\
      \mvec_{11} &|[draw,fill=blue!20]|\mvec_{42} & \mvec_{23} &  & \mvec_{1\mlen} \\
      \mvec_{31} &\mvec_{22} & \mvec_{13} & & |[draw,fill=blue!20]|\mvec_{4\mlen} \\
    };
    \node[left of=db2, left=-4pt] {$\dbmsg$};

    % \node[database,right of=db1] (db2) {$\dbmsg$};
    \node[func,below of=db1,anchor=north,above=8pt,left=8pt] (gu) {GetUser};
    \node[func,right of=gu,anchor=east,right=-5pt] (fm) {FindMatches};
    \node[func,below of=db1,anchor=east,below=2em,right=-3pt] (recover) {Recover};

    \draw[->,blue!50,thick] (user.north) |- node[black,near end,above]{$u, \mvec$} node[black,near end,below,font=\small]{register} 
    (msketch.west);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$u, \sketchval$} (db1);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$\mvec$} (db2);

    \draw[->,blue!50,thick] (user.south) |- ++(1,-0.9) node[black,near end,above]{$u, \mvectilde$} node[black,near end,below,font=\small]{login}   -| node[black,left,near end]{$u$}
    (gu.north);
    \draw[->,blue!50,thick] (user.south) |- ++(0,-0.9)  -- ++(3.1,0) |- node[black,near end, above]{$\mvectilde$}
    (fm.west);
    \draw[->,blue!50,thick] (db1.south) |- node[black,near end,above]{} (gu.east);
    \draw[->,blue!50,thick] (db2.south) |- node[black,near end,above]{} (fm.east);
    \draw[->,blue!50,thick] (gu.south) |- node[black,near end,above]{$\sketchval$} (recover.west);
    \draw[->,blue!50,thick] (fm.south) |- node[black,near end,above]{$\mvec'$} (recover.east);    
    \draw[->,blue!50,line width=2pt] (recover.south) -- node[black,near end,right]{$\mvec$ or $\bot$} ++(0, -0.65);
  \end{tikzpicture}
  % \rcnote{Rough sketch of the flow of the \biosketch.} 
  \caption{Diagram of multisketch as a part of an authentication service. 
  }
  \label{fig:mainflow}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> implementation.tex <==
\section{Implementation and Evaluation}
Follow up from the Trifecta paper
Can use almost exact copy.

==> methodology.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Methodology/Design}
\label{sec:methodology}

Use this section describe the main contribution of your paper. If you are
building something, describe the design of the system you built. If you are
measuring something (like the world!) then include the measurement pipeline.

This is typically the largest section in your paper. (In case of measurement the
result section might be bigger.)


Make sure you give enough details so that the reader is able to reproduce your
work.






==> old_engine_scalability.tex <==
\section{Trifecta Architecture Design}
\label{sec:trifecta}
In this section  we discuss in detail the Trifecta sharding architecture, an overview of which was provided in Section~\ref{sec:overview}. 


Overall architecture: Explains the three things and how they relate in 4-5 lines. 

\textbf{Shard block mining:}
- First, the SMR only "selects" $\kappa$ shard blocks mined on any given SMR block with the lowest hashes of VRF(peer-secret-key, SMR-block-number).
Implication: each shard gets fraction $\gamma_i/\gamma_i+\beta_i$

\textbf{Data availabilty votes}
- Second, after these are selected, the nodes play the data availability game and cast their vote as to the availability later in the SMR. Only the  SMR blocks which get a majority of votes are considered to be finalized in the ledger. (Adversary can cast invalid votes, but at least (1/2-beta)*N honest nodes have gotten the chunks. If we make the code such that any (1/2-beta)*N chunks can decode the block, we are done.) If the honest nodes find the coding error, they can post the coding-fraud-proof on the SMR.  Overhead per block = O(N)

Correctness. 

\textbf{State Commitment}
Round = G smr blocks -> universally defined across shards.
Average # Rounds = R
Anyone can challenge only once per round. You need to choose which shard you are challenging.
Honest policy: Challenge on the shard that you are on. 
Total overhead: N*R challenge postings per K state commit updates. 
    Overhead per G rounds = N*R
    Assume that within G rounds, you have processed at least 1 blocks in your own shard => Shard processing = B
    Total overhead = O(NR/(B)) of maintaining the challenge postings.
Choosing the challenge leader. 
In the last round of every state commitment, if we have VRF(block-number, shard-id, "leader") < threshold, you go to that shard and post a commitment. I can set threshold to maintain expected number of leaders constant. 

Correctness: (a) As long as each round has one honest node / shard, you get correctness \textbf{=> Can we do a probability calculation?} 

There are $\Gamma_i(t)*N$ honest nodes in shard i at that round. We need $P(\Gamma_i(t)*N > 1)$ for all t, for all i. We will get a horizon $H$ dependent bound $N > K \log (K*H / \epsilon )$. 
(b)Robust to adaptive adversary


Assume that SMR is running at a much faster scale and B is shard block length at a slower scale. State commitment is every block. Honest nodes rotate roughly, on average, every block.

  

\textbf{Resources Calculation} 
Overhead - Ratio of (resources used for the full protocol / Resource used for your own shard) - (resources used for your own shard + resource for other activities / Resource used for your own shard)

Want the following:
Resource for other activities / Resource used for your own shard.  = o(1)


SMR -> Ordered log Held by everyone
Content of log:
1) Shard block hashes. (comes with proof that you are eligible to send a hash) 
2) Shard state commitment. (comes with a proof that you are eligible to send commitment)
3) Shard state commitment challenge. (comes with a proof that you are eligible to challenge this round)
4) Data availability votes and fraud proofs for shard blocks

Shard log
1) Shard blocks ordered by SMR

\textbf{Main claim = Proof of properties} Protocol is robust to adaptive adversary and can support x throughput. 

% Organization
% 1. Trifecta sharding protocol details: 
% - Shard block mining using VRF, block commitments in SMR using hash / CMT commitments, you can choose to mine on whichever shard.
% - First, the SMR only "selects" \kappa shard blocks mined on any given SMR block with the lowest hashes of VRF(peer_secret_key, SMR_block_number).
% - Second, after these are selected, the nodes play the data availability game and cast their vote as to the availability later in the SMR. Only the  SMR blocks which get a majority of votes are considered to be finalized in the ledger. (Adversary can cast invalid votes, but at least (1/2-beta)*N honest nodes have gotten the chunks. If we make the code such that any (1/2-beta)*N chunks can decode the block, we are done.) If the honest nodes find the coding error, they can post the coding-fraud-proof on the SMR.  Overhead per block = O(N)


% - One round of Challenge takes A SMR blocks. At the beginning of the challenge period,
% VRF(peer_secret_key, SMR_block_number).
% - Periodically every E_n blocks we post a shard commitment to the SMR. 

% Another version (SK):
% Round = G smr blocks -> universally defined across shards.
% Average # Rounds = R
% Anyone can challenge only once per round. You need to choose which shard you are challenging.
% Honest policy: Challenge on the shard that you are on. 
% Total overhead: N*R challenge postings per K state commit updates. 
%     Overhead per G rounds = N*R
%     Assume that within G rounds, you have processed at least 1 blocks in your own shard => Shard processing = B
%     Total overhead = O(NR/(B)) of maintaining the challenge postings.
% Choosing the challenge leader. 
% In the last round of every state commitment, if we have VRF(block_number, shard_id, "leader") < threshold, you go to that shard and post a commitment. I can set threshold to maintain expected number of leaders constant. 

% Resources

  


% . We choose the one with the lowest hash among all nodes as the challenge leader.  


% , one peer can only  challenge once in an challenge round.



% - Alternate version:
% - STATE COMMITMENT
% - Anyone can challenge, one peer can only  challenge once in an challenge round. -- One challenge round = approximately 
% %- One challenge round = O(N) SMR blocks

% - O(log B) challenges
% - Epoch length = O(N)O(log B) rounds
% - Peers rotate every O(N)O(log B) rounds (constant shard rotation load)
% - Commitment leader election is challenging, since we cannot guarantee avg TP > O(1) during a state commitment leader election, (leader election has to happen every epoch=> cant ensure good throughput every epoch)

% - LEADER ELECTION
% - Cannot elect committee leader within a rotation window, for a single rotation window, no guarantee on what fraction of elected leaders are honest. If we elect over $O(K^2)$ rounds.




% - System issue: 
% => SMR has a randomness evolution
% -   -> indicator(VRF(SMR_Randomness(prev_block),peer_id)<global_threshold) => can propose a shard block for any shard of your choice. 
% assume VRF range is between 0 and 1

% - When you have a shard block, and want to post a commitment in the main chain, you need to include the certificate above.
% - Creates the following condition: at any block level, you can mine on only one shard => forces you to split \Gamma and \beta.
% - \Gamma_i is the fraction of honest nodes mining on i. \beta_i is the fraction of adv nodes mining on i.
% - shard_threshold(i)  = VRF_range =>  expected number of shard blocks per SMR block is (\Gamma_i+\beta_i)*N*shard_threshold
%  - Adjust shard_threshold(t) to make sure 
%  (\Gamma_i(t-1)+\beta_i(t-1))*N*shard_threshold(t) = \kappa
%  - expected number of shard blocks per SMR block at t is (\Gamma_i(t)+\beta_i(t))/  (\Gamma_i(t-1)+\beta_i(t-1))
%  -fraction of honest shard blocks at time t is
%   \Gamma_i(t) / (\Gamma_i(t)+\beta_i(t))
%   - number of honest shard blocks across time
%  (\Gamma_i(t))/  (\Gamma_i(t-1)+\beta_i(t-1))
 
 
 
- Separate protocol for challenge round leader election 
2. Component modules
- Data availability oracle requires anonymous network layer functionality (?)
- Interactive state commitment (appropriate references) 

3. Resource accounting to show near-linear scaling


Specifically, we discuss the various parameter settings in each of the constituent engines of the Trifecta architecture (see Figure~\ref{fig:overview}) and the overall resources (storage, compute, communication) used by each of the engines. Finally we compose the  resource usage  and  security guarantees of the  individual component engines and state the formal security and scaling properties of Trifecta sharding.


\subsection{Data availability engine}

The peers maintaining consensus engine are responsible for creating a log of all shards, as we have seen in section \ref{sec:general} that the shard log maintainer can be used to decouple transaction validity from ordering via the use of the deterministic validity bitmask. However, in order to create a validity bitmask, peers in the shard must have the block locally, if the honest peers in the shard are unable to receive a shard block pointed by the total order log, it will deadlock the shard ledger maintainer, this is demonstrated by the adversarial attack mentioned below.

\paragraph{Data obfuscating adversary:} Consider an adversarial miner in shard $i$ which manages to mine a block $B_{i,5}$, the adversary passes the block hash and the proof of mining to the consensus peers who order the blockhash pointer via the total order log. The adversary however never transmits the complete block to any honest peers. Consider a honest peer maintaining shard $i$, the peer used TOL to create the shard log consisting of $[B_{i,1},B_{i,2},..,B_{i,5},B_{i,6},..]$. The shard ledger cannot be created after $B_{i,4}$ since $B_{i,5}$ is not available. The honest peer cannot skip the block $B_{i,5}$ to process $B_{i,6}$ since the shard state at the start of $B_{i,6}$ is unknown. This will cause a deadlock and hurt liveness.

The attack can be averted by ensuring that consensus peers verify check-availability functionality before inserting a shard block in the total ordered log.  If the adversary tries the data obfuscation attack, the honest peers in shard $i$ can ask for the block data from consensus peers.

\paragraph{Strawman approach:} The strawman approach to use the Check-availability and store sample functionality by ensuring all consensus peers store all shard blocks. This approach however is resource intensive as it requires the communication and storage capacity of each consensus peer to increase as $O(K)$ which is not reasonable as $K$ increases. We hence use a Data availability engine called CMT \cite{CMT} to ensure scalability.

\begin{theorem}
    CMT based data availability engine can ensure soundness and agreement with check-availability and store-sample functionalities with a constant resource usage in the number of shards $K$ if $N>O(K)$.
\end{theorem}

\begin{proof}
Let us say for the erasure codes used in CMT a constant $\alpha$ fraction of the coded symbols need to be received to decode the block, and each node randomly samples a constant number of $S$ symbols uniformly at random. Let $m$ denote the number of symbols in each block. Then on average we will need samples from $N = \frac{\alpha m }{S\log(1-\alpha)} \approx O(m)$ nodes. Therefore, the number of symbols in each block $m$ also scales with the network size $N$. For a fixed target throughput in a single shard, scaling up the size of a block makes the block generation rate scale as $O(\frac{1}{N})$. Now, let us consider the communication load at a node that consists of two parts:
\begin{itemize}[leftmargin=*]
    \item \textit{Store sample cost:} A consensus peer takes $S$ symbols from each of the shard blocks in the $K-1$ foreign shards. This leads to a constant $O(\frac{S (m-1)}{N}) < O(1)$ communication rate if $N>O(K)$
    \item \textit{check-availability coding-fraud proof cost}: A consensus peer downloads $d-1$ symbols for each coding-fraud proof from a shard, which incurs a total communication rate of $O(\frac{(d-1)m}{N}) < O(1)$ if $N>O(K)$ 
\end{itemize} 
\end{proof}

\subsection{State commitment engine}

State commitment are important checkpoints to bootstrap a peer joining the shard and play a part of a trusted central lock to facilitate inter-shard transactions as observed in \cite{eth2}, \cite{wood2016polkadot}, etc. The state commitment has to obey the following two properties:
\begin{itemize}
    \item \textit{Validity:} A state commitment corresponds to a state observed after correct execution of transactions on the previous state. I.e. $S = STF(S',[T])$ where $S$ is the new state, $S'$ is the previous state, $[T]$ is the ledger between the two checkpoints and $STF$ stands for state transition function.
    \item \textit{Liveness:} A valid state commitment will eventually be posted and known the all consensus peers. In other words, liveness implies no deadlock in posting state commitments.
\end{itemize}
We design a state commitment engine that obeys the above properties as follows:

We divide blocks on the total ordered log into epochs and allow one valid state commitment per epoch per shard. The state commitment corresponds to the state on the shard ledger corresponding to the TOL block at the end of the epoch.

\paragraph{Committee Selection:} A peer committee is selected for a shard and is responsible to commit and challenge state commitments on the TOL. The peer committee is selected from a subset peers who were successful in mining a shard block with a mining threshold set lower than their typical mining threshold. Since theorem \ref{thm:dsa2} ensures a shard throughput of $h$. The committee will have $h$ fraction of honest nodes. The committee stays the same for a fixed number of epochs and it then reset and reformed by following the same process. The process of getting committee membership is represented by \textbf{Get committee membership} functionality and shares the mining with shard blocks, hence it occurs at negligible extra resource usage. The committee size is a constant and is denoted by $C_s$.

\paragraph{Submit state commitment:} A leader is selected from the peer committee based off of randomness from the consensus engine and is responsible to create a state commitment for the relevant epoch for the consensus engine. The leader sends the state commitment to all consensus peers who post on the TOL. The state commitment consists of the final state of the epoch and the state at the end of intermediate blocks on the epoch. More specifically:
\begin{enumerate}
        \item Merkle root $c_{s,\ell}$ of the end state $S_{s,\ell}$ after executing shard $s$ till \proposer level $\ell$.
        \item List of Merkle roots of states at intermediate blocks $[c_{s,\ell-w},..., c_{s,\ell-1}]$ where $c_{s,\ell-w}$ is the previous confirmed state commit.
    \end{enumerate}
The consensus peer deal with $O(K)$ such state commitments per epoch, if we want to set the resource usage on consensus peers as constant we need $E_l>O(K)$, where $E_l$ denotes epoch length.

\begin{figure}
    \centering
    \includegraphics[width = .45\textwidth]{images/commitment.pdf}
    \caption{State commitment}
    \label{fig:commitment}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width = .45\textwidth]{images/challenge1.pdf}
    \caption{Commitment challenge}
    \label{fig:challenge}
\end{figure}

\paragraph{Challenge state commitment:} The leader selected by the consensus engine may be adversarial and create an invalid state commitment, we introduce an interactive fraud proof based challenge protocol inspired from Truebit \cite{truebit} to implement a constant size challenge. The challenger selects the first intermediate state that it disagrees with, the challenge is posted in the TOL as depicted by figure \ref{fig:commitment}. The leader then replies to the challenge and an interactive fraud proof protocol begins as depicted in figure \ref{fig:challenge}. The interactions can be briefly described as follows:
\begin{enumerate}
    \item The leader posts $S_s$ intermediate states for the challenged state.
    \item The challenger responds with a number indicating the first intermediate state when the challengers view differs from the leader
    \item The game continues to the next iteration with the leader posting intermediate states for the smaller challenged state.
\end{enumerate}
The game ends when the conflict is resolved down to one transaction and that transaction is posted on the TOL to be resolved by the consensus peers. Since the consensus peer only process $O(1)$ transactions per commitment and the number of state commitments is constant in number of shards, the challenges of all shards exercises an $O(1)$ resource load on the consensus peers.

\begin{theorem}
    Interactive fraud proof based state commitment engine ensures validity and liveness of state commitments if a constant fraction (say 0.05) of nodes are only weakly adaptive to an adaptive adversary. Moreover the resource load on peers is $O(1)$ in the number of shards if $E_l>O(K)$ and $N>O(E_l)>O(K)$. 
    \label{thm:commitment}
\end{theorem}

\begin{proof}
    The term: Weakly adaptive to an adaptive adversary means that the nodes become adversarial after a delay of $\Delta_c$, whereas normal honest nodes can become adversarial instant under an adaptive adversary. The challenge protocol ensures that an invalid state commitment is never finalized on the TOL, and as long as one peer in the shard committee is honest, it will post a challenge to a state commitment hence ensuring validity. Notice that we only need one honest peer in the committee to ensure liveness, hence the constant fraction in the above theorem can be set to $O(1/C_s)$ = $O(1)$. 
    The leader election is determined from the randomness of consensus engine, hence an honest peer in the committee will be able to finalize a state commitment eventually in the TOL hence ensuring liveness.
    The state commit resource usage stated above require $E_l>O(K)$, moreover the intermediate state roots occupy $\frac{E_l}{N}<O(1)$ storage space which is ensured if $N>O(E_l)>O(K)$.
\end{proof}

\paragraph{Removing weakly adaptive constraint}: We propose an upgrade to the above protocol by using SNARK based verifiable computing to post state commitments. 

\subsubsection{Verifiable computing with snarks}
Removing the weakly altruistic assumption



==> resource_usage.tex <==
\section{Resource usage}

\begin{table}[]
\begin{tabular}{|c|c|l|}
\hline
\textbf{Task} & \textbf{Resource} & \textbf{Usage}  \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{State commitment}}  &  Compute & $\frac{K}{E_l}*((T_c*f_c*L_{ts})*(R_{valcom}*C_c) + (R_{valcom}*C_c)*R_{tru}*O(1))$  \\ \cline{2-3}
\multicolumn{1}{|c|}{} & Storage & \begin{tabular}[c]{@{}l@{}}$\frac{1}{E_{l}}$*K*($E_{lb}*R_{valcom}$\\ $ + O(1)*f_c*T_{valcom} + T_s*f_c*T_{valcom}*S_s*L_{ts}$)\end{tabular}  \\ \cline{2-3}
\multicolumn{1}{|c|}{} & Communication & = storage \\ \hline

\multirow{3}{*}{Hash pointer} & Compute & K*$f_{bs}$*O(1) \\ \cline{2-3}
 &  Storage & K*$f_{bs}*H_s$ \\ \cline{2-3}
 & Communication & K*$f_{bs}*H_s$ \\ \hline 

\multirow{3}{*}{Shard rotation} & Compute & $(T_c*f_c*L_{ts})*(R_{valcom}*C_c)$ + $(R_{valcom}*C_c)*R_{tru}*O(1)$  \\ \cline{2-3}
 & Storage & $\frac{K}{E_l}*((T_s*f_c*L_{ts})*(R_{valcom}*C_c) + (R_{valcom}*C_c)*R_{tru}*O(1)) + R_valcom*E_{lb}*O(1)$ \\ \cline{2-3}
 & Communication & $\frac{K}{E_l}*((T_s*f_c*L_{ts})*(R_{valcom}*C_c) + (R_{valcom}*C_c)*R_{tru}*O(1)) + R_valcom*E_{lb}*O(1)$ \\ \hline 
\multirow{3}{*}{CMT} & Compute & $K*log(\frac{B_s}{sym_s})*\frac{B_s}{sym_s*N}*f_{bs} + K*log(\frac{B_s}{sym_s})*(\log(1/\epsilon))*f_{bs} + 
f_{bs}*d$ \\ \cline{2-3}
 & Storage & $K*log(\frac{B_s}{sym_s})*\frac{B_s}{sym_s*N}*f_{bs} + K*log(\frac{B_s}{sym_s})*(\log(1/\epsilon))*f_{bs} + f_{bs}*d$ \\ \cline{2-3}
 & Communication & $K*log(\frac{B_s}{sym_s})*\frac{B_s}{sym_s*N}*f_{bs} + K*log(\frac{B_s}{sym_s})*(\log(1/\epsilon))*f_{bs} + f_{bs}*d$ \\ \hline
\end{tabular}
\caption{Resource usage table}
\end{table}



==> results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Evaluation}
\label{sec:eval}


The results section should have the results of your experiments and
measurements. Evaluation is the most important part of the research. Sometime
you might want to split it into more than one section depending on the type of the project.



Again make sure you give enough details so that the reader can reproduce your
evaluation. Your GitHub code is not a replacement of the details, GitHub will
perish, your paper will remain in this world for centuries to come. Of course,
you need strike a balance between mundane details vs what makes your evaluation
unique.









==> stateCommit.tex <==
\section{State Commitment}

NO LONGER IN USE 

Define the state commitment, state root posted on consensus engine\\
Need for state commitment\\
Dynamic self allocation
Inter shard communication

\subsection{Interactive Fraud proof}
Discuss Truebit like protocol
Give intuition of resource usage, only conflict transaction processed on consensus engine.

\subsection{Verifiable computing}
One or 2 paragraph verifible computing based state commitment.
Give intuition on why this scales.



==> trifecta.tex <==
\section{Permissionless \tfp Architecture}
We have demonstrated 
 full scaling properties of \tfp and strong security against a fully adaptive adversary this far in the {\em permissioned} setting, where the number of participants and their identity is fixed. In this section we explore how to extend \tfp sharding (and its scaling and security properties) to the permissionless setting. An obvious extension of \tfp is to permissionless proof-of-stake (PoS) systems. Here all that really needs to be done is to replace the underlying State Machine Replication with a proof-of-stake system like Algorand \cite{gilad2017algorand} rather than a permissioned system; we think of each coin as a permission token and  the results can be translated with relative ease to the PoS setting.
 
 
 Here, we specifically focus on the proof of work (PoW) setting and consider how \tfp can serve as a sharding architecture for public PoW blockchains like Bitcoin \cite{} and Ethereum \cite{}. \tfp specifically avoids identity management, so the design is a natural fit to the permissionless nature of PoW blockchains. The key question is how to integrate the permissioned \tfp architecture into a PoW blockchain. 
 
 A natural approach is  to elect a committee of PoW mining participants from within the part of the blockchain that has reached consensus and this committee serves as the participants of the permissioned \tfp architecture. One way to achieve this is via  the hybrid consensus approach \cite{hybrid}: the committee consists of a set of successive miners that are deep enough in the longest chain. The security property of the longest chain protocol ensures that all honest participants have consensus on the committee members (if the participants are embedded deep enough). The liveness property of the longest chain ensures that new miners earn the right to propose blocks on the longest chain and the chance of a  mining participant earning committee membership is directly  proportional to its hashing power in the PoW blockchain. The key vulnerability,  however, is that this approach is {\em not robust against adaptive adversaries}: this is because the committee members are known in advance and critically vulnerable in the  adaptive adversary setting (corruptible by a coordinating adversary, or self-agency to turn adversarial). Thus we look for an alternative approach to integrate \tfp sharding -- this is the focus of this section where we fix the PoW blockchain to the longest chain protocol for concreteness. 
 
 The key design aspect involves a {\em shared} mining process, followed by all participants mining  shard blocks as well as core consensus engine blocks: a {\em cryptographic sortition} ensures that the shared mining process followed by all nodes splits randomly into different roles -- the mined block becomes either a consensus engine block or one of the shard blocks. In our discussion below, we refer to the longest chain in the consensus engine  as the {\em proposal chain} and corresponding blocks in the longest chain as   {\em proposer} blocks; as is typical in longest chain protocols, confirmation of proposal blocks is based on how deep they are embedded on the longest chain. Each shard block has an identifier specifying which of the $K$ shards it belongs to. 
The proposer blocks have {\em reference links} to shard blocks (implemented via including the hash of the shard blocks inside the proposal block) -- this design is a common throughput scaling mechanism  in PoW  protocols \cite{}.  Figure \ref{fig:tflc} illustrates the overall architecture.  
The shared mining process is described in some detail below; the full pseudocode of the mining operation is in   Appendix \ref{app:alg}. 

\begin{figure}
    \centering
    \includegraphics[width = .48\textwidth]{images/\tfpLongestChain.pdf} 
    \caption{\tfp Longest chain.  }
    \label{fig:tflc}
\end{figure}

 The environment is initialized with a Genesis block for the proposer chain. Every miner mines  a ``super block" over the Genesis, comprising of information proposer block and a block for one of the $m$ shards {\em simultaneously}. This is ensured using {\em cryptographic sortition}. Each miner mines a block header which consists of data from both \proposer and shard blocks. After the miner is successful in mining the block, it selectively passes the payload based on the type of block mined, i.e., if a \proposer block is mined, the miner broadcasts the block header along with payload consisting shard block pointers while dumping the shard block payload, vice versa if a shard block is mined. The sortition happens as follows, if $0 \leq block.hash() < \tau_1$ \proposer block is mined and if $\tau_p \leq block.hash() < \tau_{s,i}$, a shard block of $i$ is mined. $\tau_p$ controls the mining rate on the proposer chain and $\tau_{s,i}-\tau_p$ controls the mining rate on the shard chain. We call the protocol based on this architecture as \tfp Longest Chain. 
The key result is that 


